Singular and Plural Functions for Functional Logic Programming

Functional logic programming (FLP) languages use non-terminating and non-confluent constructor systems (CS's) as programs in order to define non-strict non-determi-nistic functions. Two semantic alternatives have been usually considered for parameter passing with this kind of functions: call-time choice and run-time choice. While the former is the standard choice of modern FLP languages, the latter lacks some properties---mainly compositionality---that have prevented its use in practical FLP systems. Traditionally it has been considered that call-time choice induces a singular denotational semantics, while run-time choice induces a plural semantics. We have discovered that this latter identification is wrong when pattern matching is involved, and thus we propose two novel compositional plural semantics for CS's that are different from run-time choice. We study the basic properties of our plural semantics---compositionality, polarity, monotonicity for substitutions, and a restricted form of the bubbling property for constructor systems---and the relation between them and to previous proposals, concluding that these semantics form a hierarchy in the sense of set inclusion of the set of computed values. We have also identified a class of programs characterized by a syntactic criterion for which the proposed plural semantics behave the same, and a program transformation that can be used to simulate one of them by term rewriting. At the practical level, we study how to use the expressive capabilities of these semantics for improving the declarative flavour of programs. We also propose a language which combines call-time choice and our plural semantics, that we have implemented in Maude. The resulting interpreter is employed to test several significant examples showing the capabilities of the combined semantics. To appear in Theory and Practice of Logic Programming (TPLP)

==> core.tex <==
%!TEX root = plural_journal.tex

\subsection{Signature}\label{subsec:signature}
\todo{Esta seccion es bastante espesa, si se alarga la implementacion es una
buena candidata a ser borrada}

We describe in this section the signature of the modules introduced by the user.
This signature is defined in the \verb"PLURAL-SIGN" module:

{\codesize
\begin{verbatim}
fmod PLURAL-SIGN is
\end{verbatim}
}

The sort \verb"@Input@" defines all the possible data that can be introduced
by the user, being \verb"@Command@" a particular case of this input:

{\codesize
\begin{verbatim}
  sorts @Input@ @Command@ .
  subsort @Command@ < @Input@ .
\end{verbatim}
}

We define now the components of the modules introduced by the user. \verb"@Token@"
symbolizes any possible quoted identifier, that is a concrete case of expression.
The syntax \verb"_,_" builds lists of expressions, and we obtain functions with
parameters by using brackets (syntax \verb"_`(_`)"). The arrow \verb"->" constructs
rules, that are put together by juxtaposition (syntax \verb"__"):

{\codesize
\begin{verbatim}
  sorts @Token@ Exp ExpList Rule Decl StmntList Module .
  subsort @Token@ < Exp .
  subsort Exp < ExpList .
  subsort Rule < StmntList .
  subsort Decl < StmntList .
  subsort Module < @Input@ .
  
  op _,_ : ExpList ExpList -> ExpList [assoc prec 25] .
  op _`(_`) : @Token@ ExpList -> Exp [prec 10] .
  
  op _->_. : Exp Exp -> Rule [prec 30] .
  op _is_. : @Token@ @Token@ -> Decl [prec 30] .
  
  op __ : StmntList StmntList -> StmntList [comm assoc prec 35] .
\end{verbatim}
}

The predefined functions \verb"_?_" and \verb"if_then_" are also defined
here:

{\codesize
\begin{verbatim}
  op _?_ : Exp Exp -> Exp [assoc comm prec 15] .
  op if_then_ : Exp Exp -> Exp [prec 20] .
\end{verbatim}
}

We show now the syntax of the commands:

\begin{itemize}

\item Modules are introduced with syntax \verb"plural_is_endp", that expects
a token (the module identifier) and a list of rules:

{\codesize
\begin{verbatim}
  op plural_is_endp : @Token@ StmntList -> Module .
\end{verbatim}
}

\item The command \texttt{eval} evaluates the expression to obtain a value:

{\codesize
\begin{verbatim}
  op eval_. : Exp -> @Command@ .
  op eval`[depth=_`]_. : @Token@ Exp -> @Command@ .
\end{verbatim}
}

\item The command \texttt{more} demands a new value from the last
evaluated expression:

{\codesize
\begin{verbatim}
  op more`. : -> @Command@ .
\end{verbatim}
}

\item The commands \texttt{path on} and \texttt{path off} activate and deactivate
the path:

{\codesize
\begin{verbatim}
  op path`on`. : -> @Command@ .
  op path`off`. : -> @Command@ .
\end{verbatim}
}

\item The command \texttt{show path} prints the path to the last solution:

{\codesize
\begin{verbatim}
  op show`path`. : -> @Command@ .
\end{verbatim}
}

\item The command \texttt{reboot} to restarts the tool:

{\codesize
\begin{verbatim}
  op reboot`. : -> @Command@ .
\end{verbatim}
}

\item The commands \texttt{depth-first} and \texttt{width-first} allow to
change the search strategy:

{\codesize
\begin{verbatim}
  op depth-first`. : -> @Command@ .
  op breadth-first`. : -> @Command@ .
\end{verbatim}
}

\item The command \texttt{help} prints a help message:

{\codesize
\begin{verbatim}
  op help`. : -> @Command@ .
\end{verbatim}
}

\item The rule \texttt{showTr} prints the program resulting after the transformation:

{\codesize
\begin{verbatim}
  op showTr`. : -> @Command@ .
endfm
\end{verbatim}
}

\end{itemize}

The module \texttt{META-PLURAL-SIGN} defines the meta-module \texttt{SGRAMMAR}
with the signature shown above, as well as the definition of the tokens. We will
parse the terms introduced by the user with this module:

{\codesize
\begin{verbatim}
fmod META-PLURAL-SIGN is
  inc META-LEVEL .

  op SGRAMMAR : -> FModule .
  eq SGRAMMAR
    = (fmod 'SGRAMMAR is
         including 'QID-LIST .
         including 'PLURAL-SIGN .
         sorts none .
         none
         op 'token : 'Qid -> '@Token@ 
              [special(
                (id-hook('Bubble, '1 '1)
                 op-hook('qidSymbol, '<Qids>, nil, 'Qid)
                 id-hook('Exclude, '`[ '`] '< 'to ': '`, '. '`( '`)  '| )))] .
         none
         none
      endfm) .
endfm
\end{verbatim}
}


==> proofs.tex <==
%!TEX root = plural_journal.tex

When performing proofs by induction we will usually use IH to refer to the induction hypothesis of the current induction. We will also use the following auxiliary result.

\begin{lemma}\label{lSimplePropPCRWL}
For any program, $t, t' \in \CTerm_\perp$, $e \in \Exp_\perp$, $\sigma, \sigma' \in \Subst_\perp$
\begin{enumerate}
% \item $\prog \pps t \cltop t$ and $\prog \vdbp t \cltop t$  Consecuencia del item siguiente
 \item %$\prog \pps t \cltop t'$ iff $t' \ordap t$; $\prog \vdbp t \cltop t'$ iff $t' \ordap t$.
We have that $\prog \pps t \cltop t'$ iff $t' \ordap t$, and also $\prog \vdbp t \cltop t'$ iff $t' \ordap t$.
 \item If $\sigma \ordap \sigma'$ then $e\sigma \ordap e\sigma'$.
\end{enumerate}
\end{lemma}
\begin{proof}%~
%\todo{revisar demo para q se justifique la parte de \bpcrwl\ tb}
\begin{enumerate}
\item By a simple induction on the structure of $t$
% \item Assume $\prog \pps t \cltop t'$, we can prove $t' \ordap t$ by a simple induction on the structure of $t$. For the converse implication assume $t' \ordap t$, then $t \cltop t$ by the previuos item, hence $t \cltop t'$ by Lemma \ref{LMonPlural}.
 \item A simple induction on the structure of $e$.
\end{enumerate}
\end{proof}

\subsection{For Section \ref{sec:pl_sem}}
\begin{proof}[Proof for Lemma \ref{lemIntCjtoCsus}]\label{PROOFlemIntCjtoCsus}
We will prove both inclusions. 
First, to prove $\dom(?\{\theta_1 \ldots \theta_n\}) \subseteq \bigcup_i \dom(\theta_i)$ consider some $X \not\in \bigcup_i \dom(\theta_i)$, then $\rho_1 \ldots \rho_m \equiv \empsec$ and $?\{\theta_1 \ldots \theta_n\}(X) \equiv X$, hence $X \not\in \dom(?\{\theta_1 \ldots \theta_n\})$. 
% Esto era para la def de antes Now, to prove $\bigcup_i dom(\theta_i) \subseteq dom(?(\theta_1 \ldots \theta_n))$, let us consider some $X \in \bigcup_i dom(\theta_i)$. Then $\exists \theta_i \in \{\theta_1, \ldots, \theta_n\}$ such that $X \in dom(\theta_i)$. But that implies $\rho_1 \ldots \rho_m \not\equiv \empsec$, thus $?(\theta_1 \ldots \theta_n)(X) \not\equiv X$ and $X \in dom(?(\theta_1 \ldots \theta_n))$.
Now, to prove $\bigcup_i \dom(\theta_i) \subseteq \dom(?\{\theta_1 \ldots \theta_n\})$, let us consider some $X \in \bigcup_i \dom(\theta_i)$. Then $\exists \theta_i \in \{\theta_1, \ldots, \theta_n\}$ such that $X \in \dom(\theta_i)$. But that implies $\rho_1 \ldots \rho_m \not\equiv \empsec$, thus $X~?~\rho_1(X) ~?~ \ldots ~?~ \rho_m(X) \not\equiv X$ and so $?\{\theta_1 \ldots \theta_n\}(X) \not\equiv X$, because $\theta_1(X) ~?~ \ldots ~?~ \theta_n(X) \not\equiv X$ anyway. Therefore $X \in \dom(?\{\theta_1 \ldots \theta_n\})$.
\end{proof}


Theorem \ref{lCompPS} is based upon the following facts concerning the conmutativity, associativity of $?$, and the idempotence of the partial application of $?$.
 \begin{lemma}\label{lAuxCompPS2}\label{lAuxCompPS}
 For any program, $\con \in \Cntxt$ and $e_1, e_2, e_3 \in \Exp_\perp$:
 \begin{enumerate}
  \item $\denp{\con[e_1~?~e_2]} = \denp{\con[e_2~?~e_1]}$
  \item $\denp{\con[(e_1~?~e_2)~?~e_3]} = \denp{\con[e_1~?~(e_2~?~e_3)]}$
  \item $\denp{\con[e_1~?~e_1]} = \denp{\con[e_1]}$
  \item $\denp{\con[e_1]} \subseteq \denp{\con[e_1~?~e_2]}$. As a consequence, for any pair of finite chains $a_1 \ldots a_n \in \Exp_\perp^*$, $b_1 \ldots b_m \in \Exp_\perp^*$ if $\{a_1, \ldots, a_n\} \subseteq \{b_1, \ldots, b_m\}$ then for any context $\con$ $\denp{\con[a_1~?~\ldots~?~a_n]} \subseteq \denp{\con[b_1~?~\ldots~?~b_m]}$.
 \end{enumerate}
 \end{lemma}
\begin{proof}
\begin{enumerate}
 \item We have to prove that for any $t \in \CTerm_\perp$ if $\con[e_1~?~e_2] \cltop t$ then $\con[e_2~?~e_1] \cltop t$ and vice versa. This can be easily done with a simple induction on the size of the proof which acts as hypothesis.
 \item Similar to the previous item.
 \item Similar to the previous item.
 \item Assume $\con[e_1] \cltop t$, we can prove that then $\con[e_1~?~e_2] \cltop t$ with a simple induction on the size of the proof for $\con[e_1] \cltop t$. Regarding the second part of this item, assume $\con[a_1~?~\ldots~?~a_n] \cltop t$, then by the previuos items we may eliminate repeated elements in the chains and arrange them in way such that $b_1 \ldots b_m \equiv a_1 \ldots a_n b'_1 \ldots b'_k$ with $n+k=m$. Then by the first part of this item 
$$
\begin{array}{ll}
\denp{\con[a_1~?~\ldots~?~a_n]} \subseteq \denp{\con[a_1~?~\ldots~?~a_n~?~b'_1]} \\
\subseteq \ldots \subseteq \denp{\con[a_1~?~\ldots~?~a_n~?~b'_1~?~\ldots~?~b'_k]} = \denp{\con[b_1~?~\ldots~?~b_m]}
\end{array}
$$
%, 
and this process ends because both chains are finite.
\end{enumerate}
\end{proof}

\begin{proof}[Proof for Theorem \ref{lCompPS}]\label{PROOFlCompPS}
First we will prove that for any $t \in \CTerm_\perp$, if $\con[e] \cltop t$ then $\exists \{s_1, \ldots, s_n\} \subseteq \denp{e}$ such that $\con[s_1~?~\ldots~?~s_n] \cltop t$, we proceed by induction on the size $K$ of the proof for $\con[e] \cltop t$.%, measured as the number of rules of the calculus applied.
\begin{description}
 \item[Base cases] $K=1$ : 
\begin{description}
 \item[B] Then we can take $\{s_1, \ldots, s_n\} =\{\perp\}$ to do $\con[\perp] \cltop \perp$, by \textbf{B}.
 \item[RR, DC] These cases correspond to $X \cltop X$ by \crule{RR} and $c \cltop c$ by \crule{DC}. Then $\con = []$ and so the hypothesis was $e \equiv \con[e] \cltop t$. Hence we can take $\{s_1, \ldots, s_n\} = \{t\}$ to do $\con[s_1~?~\ldots~?~s_n] \equiv [t] \equiv t \cltop t$, by Lemma \ref{lSimplePropPCRWL}.
 \end{description}
 \item[Inductive steps] $K>1$ : 
\begin{description}
 \item[\crule{DC}] If $\con = []$ then we are done like in the previous step. Otherwise we have:
$$
\infer[\crule{DC}]{\con[e] \equiv c(e_1, \ldots, \con'[e], \ldots, e_l) \cltop c(t_1, \ldots, t', \ldots, t_l) \equiv t}
          {
        e_1 \cltop t_1
   & \ldots
   & \con'[e] \cltop t'
   & \ldots
   &  e_l \cltop t_l
           }
$$
Then by IH $\exists \{s_1, \ldots, s_n\} \subseteq \denp{e}$ such that $\con'[s_1~?~\ldots~?~s_n] \cltop t'$, therefore we can build the following proof:
% \begin{scriptsize}
$$
\scalebox{.93}{
\infer[\crule{DC}]{\con[s_1~?~\ldots~?~s_n] \equiv c(e_1, \ldots, \con'[s_1~?~\ldots~?~s_n], \ldots, e_l) \cltop c(t_1, \ldots, t', \ldots, t_l) \equiv t}
          {
%     \infer[]{e_1 \cltop t_1}{\hypothesis}
   e_1 \cltop t_1
   & \ldots
%    \ \infer[]{\con'[s_1~?~\ldots~?~s_n] \cltop t'}{IH}
   & \con'[s_1~?~\ldots~?~s_n] \cltop t'
   & \ldots
%   \  \infer[]{e_l \cltop t_l}{\hypothesis}
   &  e_l \cltop t_l
           }
}
$$
% \end{scriptsize}
 \item[\mbox{\apor}] If $\con = []$ then we are done like in the previous step. Otherwise we have:
$$
\scalebox{.94}{
\infer[\crule{\apor}]{\con[e] \equiv f(e_1, \ldots, \con'[e], \ldots, e_l) \cltop t}
          {
\begin{array}{c}
		e_1 \cltop p_1\theta_{11} \\
	      \ \ldots \\
              \  e_1 \cltop p_1\theta_{1 m_1} \\
	\end{array}~
       \ \ldots~
       \ \begin{array}{c}
		\con'[e] \cltop p'\theta'_{1} \\
	      \ \ldots \\
              \  \con'[e] \cltop p'\theta'_{m'} \\
	\end{array}~
       \ \ldots~
       \ \begin{array}{c}
		e_l \cltop p_l\theta_{l1} \\
	      \ \ldots \\
              \  e_l \cltop p_l\theta_{l m_l} \\
	\end{array}~
       \ ~~~~\begin{array}{c}
         ~ \\
         ~ \\
         r\theta \cltop t
         \end{array}
           }
}
$$
with $\theta = ?(\theta_{11} \ldots \theta_{1 m_1}) \uplus \ldots \uplus ?(\theta'_{1} \ldots \theta'_{m'}) \uplus \ldots \uplus \ ?(\theta_{l1} \ldots \theta_{l m_l}) \uplus \thetae$ for some $(f(p_1, \ldots, p', \ldots, p_l) \tor r) \in \prog$. Then by IH for each $\theta'_i \in \{\theta'_1, \ldots, \theta'_{m'}\}$ $\exists \{s_{i 1}, \ldots, s_{i n_i}\} \subseteq \denp{e}$ such that $\con'[s_{i 1}~?~\ldots~?~s_{i n_i}] \cltop p'\theta'_i$, hence $\con'[s_{1 1}~?~\ldots$ $?~s_{1 n_1}~?~\ldots~?~s_{m' 1}~?~\ldots~?~s_{m' {n}_{m'}}] \cltop p'\theta'_i$ by Lemma \ref{lAuxCompPS}. Therefore we can take:
$$
\begin{array}{c}
\{s_1, \ldots, s_n\} = \{s_{1 1}~?~\ldots~?~s_{1 n_1}~?~\ldots~?~s_{m' 1}~?~\ldots~?~s_{m' {n}_{m'}}\} \\
a \equiv \con'[s_{1 1}~?~\ldots~?~s_{1 n_1}~?~\ldots~?~s_{m' 1}~?~\ldots~?~s_{m' {n}_{m'}}]
\end{array}
$$
% $\{s_1, \ldots, s_n\} = \{s_{1 1}~?~\ldots~?~s_{1 n_1}~?~\ldots~?~s_{m' 1}~?~\ldots~?~s_{m' {n}_{m'}}\}$ and $a \equiv \con'[s_{1 1}~?~\ldots~?~s_{1 n_1}~?~\ldots~?~s_{m' 1}~?~\ldots~?~s_{m' {n}_{m'}}]$, 
to build the following proof:
$$
\infer[\crule{\apor}]{\con[s_1~?~\ldots~?~s_n] \equiv f(e_1, \ldots, a, \ldots, e_l) \cltop t}
          {
\begin{array}{c}
		e_1 \cltop p_1\theta_{11} \\
	      \ \ldots \\
              \  e_1 \cltop p_1\theta_{1 m_1} \\
	\end{array}~
       \ \ldots~
       \ \begin{array}{c}
		a \cltop p'\theta'_{1} \\
	      \ \ldots \\
              \  a \cltop p'\theta'_{m'} \\
	\end{array}~
       \ \ldots~
       \ \begin{array}{c}
		e_l \cltop p_l\theta_{l1} \\
	      \ \ldots \\
              \  e_l \cltop p_l\theta_{l m_l} \\
	\end{array}~
       \ ~~~~\begin{array}{c}
         ~ \\
         ~ \\
         r\theta \cltop t
         \end{array}
           }
$$
 \end{description}
\end{description}
Now we have to prove the other implication, that is, given $\{s_1, \ldots, s_n\} \subseteq \denp{e}$ such that $\con[s_1~?~\ldots~?~s_n] \cltop t$ then $\con[e] \cltop t$. If $\con = []$ then the hypothesis is $s_1~?~\ldots~?~s_n \cltop t$, so it must exists some $s_i \in \{s_1, \ldots, s_n\}$ such that $s_i \cltop t$. But then $t \ordap s_i$ by Lemma~\ref{lSimplePropPCRWL}, as $s_i \in CTerm_\perp$, as it is a value for $e$. But then the hypothesis $e \cltop s_i$ and $t \ordap s_i$ implies $e \cltop t$ by the monotonicity of Proposition \ref{LMonPlural}.\\
To prove the case when $\con\not=[]$ we need to do a simple induction on the size of $\con[s_1~?~\ldots~?~s_n] \cltop t$, in which we will not assume $\con\not=[]$. %\todoLong{Escribirlo si da tiempo, pero no tiene dificultad, en realidad esta es la parte de la implicación que se cumple incluso para reescritura}
% The base cases of this induction correspond to bases when $\con=[]$, covered by the previous case, \todo{pesado de escribir, la induccion es como la de la implicacion anterior}
\end{proof}

\begin{proof}[Proof for Proposition \ref{LMonPlural}]\label{PROOFLMonPlural}
By induction on the structure of $e \cltop t$.
\begin{description}
 \item[Base cases]~
\begin{description}
 \item[B] $e \cltop \perp \equiv t$. Then $t' \ordap t$ implies $t' \equiv \perp$, so $e' \cltop \perp \equiv t'$, by $\crule{B}$.
 \item[RR] $e \equiv X \cltop X \equiv t$. Then $t' \ordap t$ implies $t' \equiv \perp$ or $t' \equiv X$. In the first case we proceed like in the case for $\crule{B}$, in the latter as $X \equiv e \ordap e'$ implies $e' \equiv X$, so $e' \equiv X \cltop X \equiv t'$ by $\crule{RR}$.
 \item[DC] $e \equiv c \cltop c \equiv t$. Very similar to the case for $\crule{RR}$. %We can proceed in similar way we did in the previous case.
\end{description}
 \item[Inductive steps]~
\begin{description}
 \item[DC] Then we have
$$
\infer[\crule{DC}]{e \equiv c(e_1, \ldots, e_n) \cltop c(t_1, \ldots, t_n) \equiv t}
          {
            e_1 \cltop t_1
  & \ldots
  &         e_n \cltop t_n
           }
$$
Then $t' \ordap t$ implies $t' \equiv \perp$ or $t' \equiv c(t'_1, \ldots, t'_n)$ with $t'_i \ordap t_i$ for every $i \in \{1, \ldots, n\}$. In the first case we proceed like in the case for $\crule{B}$, in the latter as $c(e_1, \ldots, e_n) \equiv e \ordap e'$ implies $e' \equiv c(e'_1, \ldots, e'_n)$ with $e_i \ordap e'_i$ for every $i \in \{1, \ldots, n\}$ then by IH we get $e'_i \cltop t'_i$ for every $i \in \{1, \ldots, n\}$, and we can build the following proof:
$$
\infer[\crule{DC}]{e' \equiv c(e'_1, \ldots, e'_n) \cltop c(t'_1, \ldots, t'_n) \equiv t'}
          {e'_1 \cltop t_1 &
           \ldots &
           e'_n \cltop t_n
           }
$$
 \item[\mbox{\apor}] Then we have
$$
\infer[\crule{\apor}]{e \equiv f(e_1, \ldots, e_n) \cltop t}
          {
	\begin{array}{c}
		e_1 \cltop p_1\theta_{11} \\
	      \ \ldots \\
              \  e_1 \cltop p_1\theta_{1 m_1} \\
	\end{array}~
       \ \ldots~
       \ \begin{array}{c}
		e_n \cltop p_n\theta_{n1} \\
	      \ \ldots \\
              \  e_n \cltop p_n\theta_{n m_n} \\
	\end{array}~
       \ ~~~~\begin{array}{c}
         ~ \\
         ~ \\
         r\theta \cltop t
         \end{array}
          }
$$
with $\theta = ?(\theta_{11} \ldots \theta_{1 m_1}) \uplus \ldots \uplus \ ?(\theta_{n1} \ldots \theta_{n m_n}) \uplus \thetae$, for some $(f(p_1, \ldots, p_n) \tor r)\in \prog$. Then as $f(e_1, \ldots, e_n)$ $\equiv e \ordap e'$ implies $e' \equiv f(e'_1, \ldots, e'_n)$ with $e_i \ordap e'_i$ for every $i \in \{1, \ldots, n\}$ then by IH $\forall i \in \{1, \ldots, n\}, \forall j \in \{1, \ldots, m_i\}~e'_i \cltop p_i\theta_{i j}$. We can also apply the IH to get $r\theta \cltop t'$, as $t' \ordap t$ by hypothesis, and build the following proof:
$$
\infer[\crule{\apor}]{e' \equiv f(e'_1, \ldots, e'_n) \cltop t'}
          {
	\begin{array}{c}
		e'_1 \cltop p_1\theta_{11} \\
	      \ \ldots \\
              \  e'_1 \cltop p_1\theta_{1 m_1} \\
	\end{array}~
       \ \ldots~
       \ \begin{array}{c}
		e'_n \cltop p_n\theta_{n1} \\
	      \ \ldots \\
              \  e'_n \cltop p_n\theta_{n m_n} \\
	\end{array}~
       \ ~~~~\begin{array}{c}
         ~ \\
         ~ \\
         r\theta \cltop t'
         \end{array}
          }
$$
\end{description}
\end{description}
\end{proof}

Some of the following interesting facts about the preorders $\pordap$ and $\dsord$ will be used in the proof for Proposition \ref{LMonSusPlural}.
%Some facts about the preorders $\pordap$ and $\dsord$:
\begin{proposition}\label{LPropsOrds}%~
\begin{enumerate}
   \item $\forall \theta, \theta' \in \CSubst_\perp$, $\theta \ordap \theta'$ iff $\theta \pordap \theta'$.
%    \item Given $\theta, \theta' \icsus$, $\theta \ordap \theta'$ does not imply $dom(\theta) = dom(\theta')$.
  \item $\pordap \subseteq \icsus \times \icsus$ is a preorder but not a partial order.
  \item Given $\theta, \theta' \in \icsus$ if $\theta \pordap \theta'$ then $\theta \dsord \theta'$
   \item $\dsord \subseteq \Subst_\perp \times \Subst_\perp$ is a preorder but not a partial order
\end{enumerate} 
\end{proposition}
\begin{proof}%~
\begin{enumerate}
 \item By definition.
%  \item A simple consequence of previous item combined with first item.
 \item It is very easy to check that it is reflexive and transitive, but it is not antisymetric, as $[X/0] \pordap [X/0~?~0]$, $[X/0~?~0] \pordap [X/0]$ but $[X/0] \not= [X/0~?~0]$.
 \item  For any $X \in \var$, if $\theta(X) = t_1~?~\ldots~?~t_n$ and $\theta'(X) = t'_1~?~\ldots~?~t'_m$ (note that $\theta(X)$ has that shape even when $X \not\in dom(\theta)$, as $X$ has that shape) and $\theta(X) \clto t$ then it must exist some $t_i \in \{t_1, \ldots, t_n\}$ such that $t_i \clto t$, and so $t \ordap t_i$ by Lemma \ref{lSimplePropPCRWL}. But then $t \ordap t_i \ordap t'_j$ for some $t_j \in \{t'_1, \ldots, t'_m\}$, because $\theta \pordap \theta'$, hence $t'_j \clto t$ by Lemma \ref{lSimplePropPCRWL} and so $\theta'(X) \clto t$.
% . But then $t'_j \clto t$ by Lemma \ref{LMonPlural} and so $\theta'(X) \clto t$.
 \item It is very easy to check that it is reflexive and transitive, but it is not antisymetric, because given $\prog = \{f \tor 1, g \tor 1\}$ we have $[X/f] \dsord [X/g]$ and $[X/g] \dsord [X/f]$ while $[X/f] \not= [X/g]$.
\end{enumerate}
\end{proof}


The following standard notions from term rewriting \cite{baader-nipkow} will also be used in the proof for Proposition \ref{LMonSusPlural}.
\begin{definition}\label{DefAuxCon}
 \begin{itemize}
  \item The set of positions of an expression $e$ is the set $\pos{e}$ of strings over the alfabet of positive integers defined as $\pos{X} = \{\epsilon\}$, if $X \in \var$; $\pos{h(e_1, \ldots, e_n)} = \{\epsilon\} \cup \bigcup_{i \in \{1, \ldots, n\}} \{i.p~|~p \in \pos{e_i}\}$ otherwise, where $\epsilon$ denotes the empty string and $\_.\_$ is used for concatenation.\\
 We say that two positions are parallel if none of them is prefix of the other.
  \item For any $e \in Exp_\perp$, $p \in \pos{e}$, the subexpression of $e$ at position $p$ denoted by $s|_p$, is defined as $e|_\epsilon = e$; $h(e_1, \ldots, e_n)|_{i.q}= e_i|_q$.
  \item For any $e,e' \in Exp_\perp$, $p \in \pos{e}$, by $e[e']_p$ we denote the expression obtained from $e$ by replacing the subexpression at position $p$ by $e'$, defined as $e[e']_\epsilon = e'$; $f(e_1, \ldots, e_n)[e']_{i.q} = f(e_1, \ldots, e_i[e']_q, \ldots, e_n)$.
  \item As one-hole context can be understood as funcions $\con : Exp_\perp \rightarrow Exp_\perp$, for any $\con \in Cntx$ we may assume some $e \in Exp_\perp, p \in \pos{e}$ such that $\con = \lambda e'.e[e']_p$. With this in mind Theorem \ref{lCompPS} can be recasted as $\denp{e[e']_p} = \bigcup_{\overline{t} \subseteq \denp{e'}} \denp{e[?\overline{t}]_p}$, where $?\{t_1, \ldots, t_n\}$ denotes $t_1~?~\ldots~?~t_n$ for some arrangement of the elements of $\{t_1, \ldots,$ $t_n\}$ in $t_1~?~\ldots~?~t_n$.
 \end{itemize}
\end{definition}


\begin{proof}[Proof for Proposition \ref{LMonSusPlural}]\label{PROOFLMonSusPlural}%~
\begin{enumerate}
 \item If $e \equiv X \in \var$, assume $e\sigma \equiv \sigma(X) \cltop t$, then $e\sigma' \equiv \sigma'(X) \cltop t$ with a proof of the same size or smaller, by hypothesis. Otherwise we proceed by induction on the structure of $e\sigma \cltop t$.
\begin{description}
 \item[Base cases]~
 \begin{description}
   \item[B] Then $t \equiv \perp$ and $e\sigma' \cltop \perp$ with a proof of size $1$ just applying rule $\crule{B}$.
   \item[RR] Then $e \in \var$ and we are in the previous case.
   \item[DC] Then $e \equiv c \in \CS^0$, as $e \not\in \var$, hence $e\sigma \equiv c \equiv e\sigma'$ and every proof for $e\sigma \cltop t$ is a proof for $e\sigma' \cltop t$.
  \end{description}
 \item[Inductive steps]~
 \begin{description}
\item[DC] Then $e \equiv c(e_1, \ldots, e_n)$, as $e \not\in \var$, and we have:
$$
\infer[\crule{DC}]{e\sigma \equiv c(e_1\sigma, \ldots, e_n\sigma) \cltop c(t_1, \ldots, t_n) \equiv t}
          {
       e_1\sigma \cltop t_1
    & \ldots
    &  e_n\sigma \cltop t_n
          }
$$
By IH or the proof of the other cases $\forall i \in \{1, \ldots, n\}$ we have $e_i\sigma' \cltop t_i$ with a proof of the same size or smaller, so we can built a proof for $e\sigma' \equiv c(e_1\sigma', \ldots, e_n\sigma') \cltop c(t_1, \ldots, t_n) \equiv t$ using $\crule{D}$C, with a size equal or smaller than the size of the starting proof.
   \item[\mbox{\apor}] Very similar to the proof of the previuos case. We have $e \equiv f(e_1, \ldots, e_n)$ (as $e \not\in \var$) and given a proof for $e\sigma \equiv f(e_1, \ldots, e_n)\sigma \cltop t$, we apply the IH to every $e_i\sigma \cltop p_i\theta_{i j}$ to get that $e_i\sigma' \cltop p_i\theta_{i j}$ with a proof of the same size or smaller. But then we can use these proofs in a $\crule{\apor}$ step from $e\sigma' \equiv f(e_1\sigma', \ldots, e_n\sigma')$ and use the same substitution $\theta \in \icsus$ for parameter passing, constructing a proof with a size equal or smaller than the size of the starting one.
  \end{description}
 \end{description}
 \item If $\theta \ordap \theta'$ then for any $X \in \var$ we have $\theta(X) \ordap \theta'(X)$, hence if $\theta(X) \cltop t$ then $\theta'(X) \cltop t$ with a proof of the same size or smaller, by the polarity of \apcrwl\ from Proposition \ref{LMonPlural}. But then we can apply the strong monotonicity of $Subst_\perp$ from the previous item, to get the desired result.
  \item Using the notations of Definition \ref{DefAuxCon}, given $X_i \in \overline{X} = var(e)$ if the set of positions of the occurrences of $X_i$ in $e$ is $\{p_{i 1}, \ldots, p_{i m_i}\}$ then $e \equiv e[X_i]_{p_{i 1}} \equiv (e[X_i]_{p_{i 1}})[X_i]_{p_{i 2}} \equiv \ldots e[X_i]_{p_{i 1}}\ldots [X_i]_{p_{i m_i}}$. As the positions of any pair of different occurrences of (possibly different) variables are parallel, we can do this for every variable in $\overline{X}$ to get $e \equiv e[Y_1]_{o_1}\ldots[Y_m]_{o_m}$, where $\{o_1, \ldots, o_m\}$ is the set of positions of every occurrence in $e$ of any variable in $var(e)$ and $\{Y_1, \ldots, Y_m\} = \overline{X}$. Note how each position in $\{o_1, \ldots, o_m\}$ is parallel to each other. 
% $\{Y_1, \ldots, Y_m\} = \overline{X}$ and some parallel set of positions $\{o_1, \ldots, o_m\}$, the set of positions of every occurrence in $e$ of any variable in $var(e)$. %for $\{Y_1, \ldots, Y_m\} = \overline{X}$ and some parallel set of positions $\{o_1, \ldots, o_m\}$, the set of positions of every occurrence in $e$ of any variable in $var(e)$. 
But then we can apply the recasted version of Theorem \ref{lCompPS} that appears in Definition \ref{DefAuxCon}, to get:
$$
\begin{array}{ll}
\denp{e\sigma} = \denp{e[Y_1\sigma]_{o_1}\ldots[Y_m\sigma]_{o_m}} \\
= \bigcup\limits_{{\overline{t_1} \subseteq \denp{Y_1\sigma}}} \denp{e[?\overline{t_1}]_{o_1}\ldots[Y_m\sigma]_{o_m}} & \mbox{ by Theorem \ref{lCompPS}}\\
= \bigcup\limits_{\overline{\overline{t} \subseteq \denp{Y\sigma}}} \denp{e[\overline{?\overline{t}}]_{\overline{o}}}  & \mbox{ by Theorem \ref{lCompPS} (many times)}\\
= \bigcup\limits_{\overline{\overline{t} \subseteq \denp{Y\sigma'}}} \denp{e[\overline{?\overline{t}}]_{\overline{o}}}  & \mbox{ as } \sigma \dsord \sigma'\\
= \denp{e[Y_1\sigma']_{o_1}\ldots[Y_m\sigma']_{o_m}} = \denp{e\sigma'} & \mbox{ by Theorem \ref{lCompPS}}\\
% 
% 
% = \bigcup\limits_{\overline{\overline{t} \subseteq \denp{\sigma(X)}}} \denp{e[\overline{?\overline{t}}]} & \mbox{ by Theorem \ref{lCompPS}}\\
% \subseteq \bigcup\limits_{\overline{\overline{t} \subseteq \denp{\sigma'(X)}}} \denp{e[\overline{?\overline{t}}]} & \mbox{ as } \sigma \dsord \sigma'\\
% = \denp{e[\overline{\sigma'(X)}]} = \denp{e\sigma'} & \mbox{ by Theorem \ref{lCompPS}}\\
\end{array}
$$
% If $var(e) = \overline{X}$ then $e \equiv e[\overline{X}]$ for some many-hole context $e[]$. But then:
% $$
% \begin{array}{ll}
% \denp{e\sigma} = \denp{e[\overline{\sigma(X)}]} \\
% = \bigcup\limits_{\overline{\overline{t} \subseteq \denp{\sigma(X)}}} \denp{e[\overline{?\overline{t}}]} & \mbox{ by lemma \ref{lCompPS}}\\
% \subseteq \bigcup\limits_{\overline{\overline{t} \subseteq \denp{\sigma'(X)}}} \denp{e[\overline{?\overline{t}}]} & \mbox{ as } \sigma \dsord \sigma'\\
% = \denp{e[\overline{\sigma'(X)}]} = \denp{e\sigma'} & \mbox{ by lemma \ref{lCompPS}}\\
% \end{array}
% $$
Note that we cannot claim $e\sigma' \cltop t$ with proof of the same size of smaller, as we can see for example with $\sigma = [X/0] \dsord [X/0~?~0] = \sigma', e \equiv X, t\equiv 0$ for which $e\sigma \equiv 0 \cltop 0$ with size one but $e\sigma' \equiv 0~?~0 \cltop 0$ with size greater or equal to four.
 \item If $\theta \pordap \theta'$ then $\theta \dsord \theta'$ by Proposition \ref{LPropsOrds}, hence this item holds by the previous item. 
\end{enumerate}
\end{proof}

\begin{proof}[For Proposition \ref{lemCompAPlCCon}]\label{PROOFlemCompAPlCCon}
%\todo{mover a apendice de demos}
For the left to right inclusion we must prove that given $\vdap \ccon[e] \clto t$ then $\exists s \in \denap{e}$ such that $\vdap \ccon[s] \clto t$. We proceed by induction on the size of the \apcrwl-proof for $\vdap \ccon[e] \clto t$. Concerning the base cases:
\begin{description}
	\item[B] Then $t \equiv \perp$ and we can take $s \equiv \perp$ for which $e \clto \perp$ and $\ccon[s] \clto \perp \equiv t$ by rule \crule{B} in both cases.
   \item[RR, DC] Then either $\ccon[e] \equiv X \in \var$ or $\ccon[e] \equiv c \in \CS^0$, therefore $\ccon = []$ and thus $e \equiv \ccon[e] \clto t$ by hypothesis. But then we can take $s \equiv t$ so we have $\ccon[s] \equiv t \clto t$ by Lemma \refp{lSimplePropPCRWL}.
\end{description}
Regarding the inductive step:
\begin{description}
	\item[DC] If $\ccon = []$ we proceed like in the previous case, otherwise we have:
$$
\infer[\crule{DC}]{\ccon[e] \equiv c(e_1, \ldots, \ccon'[e], \ldots, e_n) \clto c(t_1, \ldots, t', \ldots, t_n) \equiv t}
         {
        e_1 \clto t_1
     & \ldots
     & \ccon'[e] \clto t'
     & \ldots
     & e_n \clto t_n
         }
$$
But then we can apply the IH to $\ccon'[e] \clto t'$ to get some $s \in \denap{e}$ such that $\ccon'[s] \clto t'$, so we can build the following proof:
$$
\infer[\crule{DC}]{\ccon[s] \equiv c(e_1, \ldots, \ccon'[s], \ldots, e_n) \clto c(t_1, \ldots, t', \ldots, t_n) \equiv t}
         {
        \infer{e_1 \clto t_1}{\hypothesis}
     & \ldots
     & \infer{\ccon'[s] \clto t'}{IH}
     & \ldots
     & \infer{e_n \clto t_n}{\hypothesis}
         }
$$
   \item[\apor] If $\ccon = []$ we proceed like in the previous case, otherwise we have $\ccon = f(e_1, \ldots, \ccon', \ldots, e_n)$ for some $f \in FS$, which contradicts the hypothesis as $\ccon$ should be a c-context, so we are done.
\end{description}

Now, to prove the converse inclusion, we have to prove that given some $s \in \denap{e}$ such that $\vdap \ccon[s] \clto t$ then $\vdap \ccon[e] \clto t$. If $\ccon = []$ then we have $s \equiv \ccon[s] \clto t$, and so $t \ordap s$ by Lemma \refp{lSimplePropPCRWL}. But then, as $s \in \denap{e}$, we get $\ccon[e] \equiv e \clto t$ by Proposition \refp{LMonPlural}. To prove the case where $\ccon \not= []$ we proceed by induction on the size of the proof for $\vdap \ccon[s] \clto t$. Concerning the base cases:
\begin{description}
	\item[B] Then $t \equiv \perp$ and we can take $s \equiv \perp$ for which $e \clto \perp$ and $\ccon[s] \clto \perp \equiv t$ by rule B in both cases.
   \item[RR, DC] Then either $\ccon[e] \equiv X \in \var$ or $\ccon[e] \equiv c \in \CS^0$, therefore $\ccon = []$ and we proceed like in the previous case.
\end{description}
Regarding the inductive step:
\begin{description}
	\item[\crule{DC}] If $\ccon = []$ we proceed like in the previous case, otherwise we have:
$$
\infer[\crule{DC}]{\ccon[s] \equiv c(e_1, \ldots, \ccon'[s], \ldots, e_n) \clto c(t_1, \ldots, t', \ldots, t_n) \equiv t}
         {
        e_1 \clto t_1
     & \ldots
     & \ccon'[s] \clto t'
     & \ldots
     & e_n \clto t_n
         }
$$
But then we can apply the IH to $\ccon'[s] \clto t'$ with $s \in \denap{e}$ to get $\ccon'[e] \clto t'$, so we can build the following proof:
$$
\infer[\crule{DC}]{\ccon[e] \equiv c(e_1, \ldots, \ccon'[e], \ldots, e_n) \clto c(t_1, \ldots, t', \ldots, t_n) \equiv t}
         {
        \infer{e_1 \clto t_1}{\hypothesis}
     & \ldots
     & \infer{\ccon'[e] \clto t'}{IH}
     & \ldots
     & \infer{e_n \clto t_n}{\hypothesis}
         }
$$
   \item[\apor] If $\ccon = []$ we proceed like in the previous case, otherwise we have $\ccon = f(e_1, \ldots, \ccon', \ldots, e_n)$ for some $f \in FS$, which contradicts the hypothesis as $\ccon$ should be a c-context, so we are done.
\end{description}
\end{proof}

\begin{lemma}\label{lemAuxBubAPl}
Under any program and for every $e_1, e_2 \in \Exp_\perp$, $\denap{e_1~?~e_2} = \denap{e_1} \cup \denap{e_2}$.
\end{lemma}
\begin{proof}
For the left to right inclusion, assume we have $\vdap e_1~?~e_2 \clto t$, then it must be with a proof of the following shape
$$
\infer[\mbox{\apor}]{e_1~?~e_2 \clto t}
      {
      \begin{array}{l}
      e_1 \clto s_{1 1} \\
     \ldots \\
      e_1 \clto s_{1 m_1} \\
      \end{array}
   \       \begin{array}{l}
      e_2 \clto s_{2 1} \\
     \ldots \\
      e_2 \clto s_{2 m_2} \\
      \end{array}
    \ \begin{array}{l}
       ~ \\ ~ \\
       s_{i 1}~?~(s_{i 2}~?~\ldots~?~s_{i m_i}) \clto t
      \end{array}
      }
$$
As any \apcrwl-proof is finite, then either $m_i = 1$ or the proof for $\vdap s_{i 1}~?~(s_{i 2}~?~\ldots~?~s_{i m_i}) \clto t$ ends with a proof for $\vdap s \clto t$ as premise, for some $s \in \denap{s_{i j}}$ for some $j \in \{1, \ldots, m_i\}$. Anyway by Lemma \ref{lSimplePropPCRWL} we get $t \ordap s \ordap s_{i j} \in \denap{e_i}$ (with $s \equiv s_{i j}$ in case $m_i = 1$). But then $t \in \denap{e_i} \subseteq \denap{e_1} \cup \denap{e_2}$ by Proposition \ref{LMonPlural}.\\
%
Regarding the converse inclusion, assume $t \in \denap{e_i}$, then we can build the following proof:
$$
\infer[\mbox{\apor}]{~~~~~~~~~~~~~~~~~~~~e_1~?~e_2 \clto t~~~~~~~~~~~~~~~~~~~~}
     {
     \infer{e_i \clto t}{\hypothesis}
   & \infer[\crule{B}]{e_{3-i} \clto \perp}{}
   & \infer{t \clto t}{\mbox{Lemma \ref{lSimplePropPCRWL}}}
     }
$$
\end{proof}

\begin{proof}[For Lemma \ref{lemmaCompress1}]
Consider some element $(t_1, \ldots, t_n) \in \{(X_1\theta, \ldots, X_n\theta)~|~\theta \in \Theta\}$ and its corresponding $\theta \in \Theta$. We can just take $\theta_1 = \ldots = \theta_n = \theta$ to conclude that $(t_1, \ldots, t_n) \equiv (X_1\theta, \ldots, X_n\theta) \equiv (X_1\theta_1, \ldots, X_n\theta_n) \in \{X_1\theta_1\} \times \ldots \times \{X_n\theta_n\} \subseteq \{X_1\theta_1~|~\theta_1 \in \Theta\} \times \ldots \times \{X_n\theta_n~|~\theta_n \in \Theta\}$. 
%$\theta \in \Theta$, then we can take $\theta_1 = \ldots = \theta_n = \theta$ so $(X_1\theta, \ldots, X_n\theta) \in \{(X_1\theta, \ldots, X_n\theta)\} = \{X_1\theta_1\} \times \ldots \times \{X_n\theta_n\} \subseteq \{X_1\theta_1~|~\theta_1 \in \Theta\} \times \ldots \times \{X_n\theta_n~|~\theta_n \in \Theta\}$. 
\end{proof}


\subsection{For Section \ref{sect:hierarchy}}
% parece que no se usa para nada
%\begin{lemma}
%For any \crwl-program $\prog$, $e \in Exp_\perp, t\in CTerm_\perp, \theta \in CSubst_\perp$ if $\prog \pps e \cltop t$ then $\prog \pps e\theta \cltop t\theta$.
%\end{lemma}
%\begin{proof}
%If $t \equiv \perp$ then $e\theta \cltop t\theta \equiv \perp$ by B, otherwise the proof is just a simple induction over the size of $e \cltop t$.
%\end{proof}

%\begin{lemma}\label{lDenSubst2}
%For any finite not empty $\Theta \subseteq \denp{\sigma}$ we have $?\Theta \dsord \sigma$.
%\end{lemma}
\begin{proof}[Proof for Lemma \ref{lDenSubst2}]\label{PROOFlDenSubst2}
First of all $\Theta$ is required to be finite and not empty because otherwise $?\Theta$ is not defined. Given $X \in \var$ assume $\vdbp (?\Theta)(X) \clto t$ for some $t \in \CTerm_\perp$, then we have two possibilities:
\begin{enumerate}
	\item[a)] $\exists \theta_i  \in \Theta. X \not\in \dom(\theta_i)$. Then the hypothesis is $\vdbp (?\Theta)(X) \equiv X~?~\rho_1(X)~?~\ldots$ $?~\rho_m(X) \clto t$ for some $\{\rho_1, \ldots, \rho_m\} \subseteq \Theta$, and we have two possibilities: 
\begin{enumerate}
	\item[i)] If $\vdbp X \clto t$ then either $t \equiv \perp$, so $\vdap \sigma(X) \clto \perp \equiv t$ by \crule{B}; or $t \equiv X$. But then $\vdbp \sigma(X) \clto \theta_i(X) \equiv$, because $X \not\in \dom(\theta_i)$ and $\theta_i \in \Theta \subseteq \denbp{\sigma}$.
    \item[ii)] On the other hand $\vdbp \rho_j(X) \clto t$ for some $\theta_j \in \{\rho_1, \ldots, \rho_m\}$, hence $t \ordap \rho_j(X)$ by Lemma \ref{lSimplePropPCRWL}. Besides $\vdbp \sigma(X) \clto \rho_j(X)$, because $\theta_j \in \{\rho_1, \ldots, \rho_m\} \subseteq \Theta \subseteq \denbp{\sigma}$. But then  $\vdbp \sigma(X) \clto t$ by the polarity of \bpcrwl\ from Theorem \ref{ThPropsBetaPlHeredadas}. 
\end{enumerate}
    \item[b)] Otherwise $\forall \theta_i \in \Theta. X \in \dom(\theta_i)$. Then if $\Theta = \{\theta_1, \ldots, \theta_n\}$ the hypothesis is $\vdbp (?\Theta)(X) \equiv \theta_1(X)~?~\ldots$ $?~\theta_n(X) \clto t$ and so $\vdap \theta_i(X) \clto t$ for some $ \theta_i \in \Theta$, and we can proceed like in the second item of the previous case. 
\end{enumerate}
\end{proof}

% Subconjunto del lema de FSTTCS'08 que solo tiene las propiedades esenciales y adaptado para \pbcrwl
\begin{lemma}\label{lemInfDomDenSubst}
For any program $\prog$, $\sigma \in Subst_\perp$ we have that $\denbp{\sigma} \neq \emptyset$ and given $\overline{X} = \dom(\sigma)$ then $[\overline{X/\perp}] \in \denbp{\sigma}$.
\end{lemma}
\begin{proof}%~
It is enough to prove that if $\overline{X} = \dom(\sigma)$ then $[\overline{X/\perp}] \in \denp{\sigma}$. First of all $[\overline{X/\perp}] \in \CSubst_\perp$ by definition. Now consider some $Y \in \var$.
\begin{enumerate}
	\item[i)] If $Y \in \overline{X}$ then $\pps \sigma(Y) \cltop \perp \equiv Y[\overline{X/\perp}]$, by rule \crule{B}.
    \item[ii)] Otherwise $Y \not\in \overline{X} = \dom(\sigma)$, hence $\pps \sigma(Y) \equiv Y \cltop Y \equiv Y[\overline{X/\perp}]$, by rule \crule{RR}.
\end{enumerate}
\end{proof}


\begin{lemma}\label{lemIncCsubstOrd}
For any finite and not empty $\Theta, \Theta' \subseteq \CSubst_\perp$, if $\Theta \subseteq \Theta'$ then $?\Theta \pordap ?\Theta'$.
\end{lemma}
\begin{proof}
Let $\Theta = \{\theta1, \ldots, \theta_n\}$ and $\Theta' = \{\theta'_1, \ldots, \theta'_k\}$ be. Given an arbitrary $X \in \var$:
\begin{enumerate}
	\item If $\exists \theta \in \Theta. X \not\in \dom(\theta)$ then $\theta \in \Theta'$, because $\Theta \subseteq \Theta'$, which also implies that for $\rho_1, \ldots, \rho_m = \theta_1, \ldots, \theta_n~|~\lambda \theta. X \in \dom(\theta)$ and $\rho'_1, \ldots, \rho'_l = \theta'_1, \ldots, \theta'_k~|~\lambda \theta. X \in \dom(\theta)$ then $\{\rho_1, \ldots, \rho_m\} \subseteq \{\rho'_1, \ldots, \rho'_l\}$. But then
$$
\begin{array}{l}
(?\Theta)(X) = X~?~\rho_1(X)~?~\ldots~?~\rho_m(X) \\
(?\Theta')(X) = X~?~\rho'_1(X)~?~\ldots~?~\rho'_l(X) \\
\end{array}
$$
and $\{X, \rho_1(X), \ldots, \rho_m(X)\} \subseteq \{X, \rho'_1(X), \ldots, \rho'_l(X)\}$, so $?\Theta \pordap ?\Theta'$ holds for $X$ by reflexivity of $\ordap$.
\item Otherwise $\forall \theta \in \Theta. X \in dom(\theta)$ which implies $(?\Theta)(X) = \theta_1(X)~?~\ldots~?~\theta_n(X)$. But then for $\rho'_1, \ldots, \rho'_l = \theta'_1, \ldots, \theta'_k~|~\lambda \theta. X \in \dom(\theta)$ we have that $\Theta \subseteq \Theta'$ implies both $\{\theta_1(X), \ldots, \theta_n(X)\} \subseteq \{X, \rho'_1(X), \ldots, \rho'_l(X)\}$ and $\{\theta_1(X), \ldots, \theta_n(X)\} \subseteq \{\theta'_1(X), \ldots, \theta'_k(X)\}$, so $?\Theta \pordap ?\Theta'$ holds for $X$ by reflexivity of $\ordap$.
\end{enumerate}
\end{proof}

%\begin{lemma}\label{lDenSubst1}
%For any $\sigma \in Subst_\perp, e \in Exp_\perp, t \in CTerm_\perp$ if $\pps e\sigma \cltop t$ then $\exists \Theta \subseteq \denp{\sigma}$ finite and not empty such that $\pps e(?\Theta) \cltop t$
%\end{lemma}
\begin{proof}[Proof for Lemma \ref{lDenSubst1}]\label{PROOFlDenSubst1}
By a case distinction over $e$:
\begin{itemize}
 \item If $e \equiv X \in \dom(\sigma)$ : Then $e\sigma \equiv \sigma(X) \cltop t$, so we can define:
$$
\theta(Y) = \left\{\begin{array}{ll}
t & \mbox{ if } Y \equiv X \\
\perp & \mbox{ if } Y \in (\dom(\sigma) \setminus \{X\})\\
Y & \mbox{ if } Y \not\in \dom(\sigma)
\end{array} \right.
$$
Then $\theta \in \denp{\sigma}$ because obviously $\theta \in \CSubst_\perp$, and given $Z \in \var$. 
\begin{enumerate}
	\item[a)] If $Z \equiv X$ then $\pps \sigma(Z) \equiv \sigma(X) \cltop t \equiv \theta(Z)$ by hypothesis.
    \item[b)] If $Z \in (\dom(\sigma) \setminus \{X\})$ then $\pps \sigma(Z) \cltop \perp \equiv \theta(Z)$ by rule \crule{B}.
     \item[c)] Otherwise $Z \not\in \dom(\sigma)$ and then $\pps \sigma(Z) \equiv Z \cltop Z \equiv \theta(Z)$ by rule \crule{RR}.
\end{enumerate}
%Then is trivial to check that $\theta \in \denp{\sigma}$, so 
Now we can take $\Theta = \{\theta\}$ for which $e(?\Theta) \equiv \theta(X) \equiv t \cltop t$, by Lemma \ref{lSimplePropPCRWL}.%\ref{lPropPCRWL}.
 \item If $e \equiv X \not\in \dom(\sigma)$ : Then given $\overline{Y} = \dom(\sigma)$ we define $[\overline{Y/\perp}]$ for which $[\overline{Y/\perp}]\in \denp{\sigma}$ by Lemma \ref{lemInfDomDenSubst}, so we can take $\Theta = \{[\overline{Y/\perp}]\}$ for which $\denp{e\sigma} = \denp{X} = \denp{X(?\Theta)}$.
 \item If $e \not\in \var$ then we proceed by induction over the structure of $e\sigma \cltop t$:
\begin{description}
 \item[Base cases]~
 \begin{description}
  \item[B] Then $t \equiv \perp$, so given $\overline{Y} = dom(\sigma)$ we can take $\Theta = \{[\overline{Y/\perp}]\}$ for which $e(?\Theta) \cltop \perp$ by \crule{B}.
  \item[RR] Then $e \in \var$ and we are in the previous case.
  \item[DC] Similar to the case for $e \equiv X \not\in dom(\sigma)$.
 \end{description}
 \item[Inductive steps]~
  \begin{description}
   \item[DC] Then $e \equiv c(e_1, \ldots, e_n)$, as $e \not\in \var$, and we have:
$$
\infer[\crule{DC}]{e\sigma \equiv c(e_1\sigma, \ldots, e_n\sigma) \cltop c(t_1, \ldots, t_n) \equiv t}
          {
       e_1\sigma \cltop t_1
    & \ldots
    &  e_n\sigma \cltop t_n
          }
$$
By IH of the proof of the other cases $\forall i \in \{1, \ldots, n\} ~\exists \Theta_i \subseteq \denp{\sigma}$ such that $e_i(?\Theta_i) \cltop t_i$. Hence we can define $\Theta = \bigcup_{i \in \{1, \ldots, n\}} \Theta_i$, for which $\forall i \in \{1, \ldots, n\} ~?\Theta_i \pordap ?\Theta$ by Lemma \ref{lemIncCsubstOrd}, and so $\forall i \in \{1, \ldots, n\}~e_i(?\Theta_i) \cltop t_i$ implies $e_i(?\Theta) \cltop t_i$, by %Lemma \ref{LMonSusPlural}. %\ref{lPropPCRWL}. 
the monotonicity for substitutions of \bpcrwl\ from Theorem \ref{ThPropsBetaPlHeredadas}. 
Therefore $e(?\Theta) \cltop c(t_1, \ldots, t_n)$ by \crule{DC}.
   \item[\bpor] Similar to the proof of the previuos case. We also have $e \equiv f(e_1, \ldots, e_n)$ (as $e \not\in \var$) and given a proof for $e\sigma \equiv f(e_1, \ldots, e_n)\sigma \cltop t$, we apply the IH of the proof of the other cases to every $e_i\sigma \cltop p_i\theta_{i j}$ to get some $\Theta_{i j} \subseteq \denp{\sigma}$ such that $e_i(?\Theta_{i j}) \clto p_i\theta_{i j}$. Then we define $\Theta = \bigcup_{i \in \{1, \ldots, n\}}\bigcup_{j \in \{1, \ldots, m_i\}} \Theta_{i j}$ for which $\forall i, j,~ ?\Theta_{ i j} \pordap ?\Theta$ %obviously holds
by Lemma \ref{lemIncCsubstOrd}, and as a consequence $\forall i, j,~ e_i(?\Theta) \cltop p_i\theta_{i j}$. Hence with $e(?\Theta) \equiv f(e_1(?\Theta), \ldots, e_n(?\Theta))$ we can compute the same value for its arguments and thus use the same compressible substitution $\theta \in \icsus$ for parameter passing in \bpor, employing the same $\theta_e \in \icsus$ to instantiate the extra variables.
  \end{description}
\end{description}
\end{itemize}
\end{proof}


\begin{proof}[Proof for Proposition \ref{LemPropsCC1}]\label{PROOFLemPropsCC1}
\begin{enumerate}
	\item[a)] By definition, as $\Theta \subseteq \CSubst_\perp$ and is also finite.
    \item[b)] Assuming $\Theta \subseteq \cc{\Theta}$ then $?\Theta \pordap ?\cc{\Theta}$ holds by %definition of $?$ and $\pordap$
Lemma \ref{lemIncCsubstOrd}. So all that is left is proving that $\Theta \subseteq \cc{\Theta}$. Conside some $\theta \in \Theta$, then $\dom(\theta) \subseteq \{X_1, \ldots, X_n\}$ by definition of $\{X_1, \ldots, X_n\}$, hence $\theta = [X_1\theta, \ldots, X_n\theta] \in \cc{\Theta}$, by definition of $\cc{\Theta}$, as $\theta \in \Theta$.
     \item[c)] For any $\mu \in \cc{\Theta}$ we have that $\mu = [X_1/X_1\theta_1, \ldots, X_n/X_n\theta_n]$ for some $\theta_1, \ldots, \theta_n \in \Theta$, by definition of $\cc{\Theta}$. Therefore $dom(\mu) \subseteq \{X_1, \ldots, X_n\}$, thus $\bigcup_{\mu \in \cc{\Theta}}dom(\mu)$ $\subseteq \{X_1, \ldots, X_n\}$.\\
Regarding the converse inclusion, given some $X_1 \in \{X_1, \ldots, X_n\}$ by definition of $\{X_1, \ldots, X_n\}$ then $\exists \theta\in \Theta$ such that $X_i \in \dom(\theta)$, thus $\theta(X_i) \not\equiv X_i$. Moreover $[X_1/X_1\theta, \ldots, X_i/X_i\theta, \ldots, X_n/X_n\theta] \in \cc{\Theta}$, by definition of $\cc{\Theta}$, and $[X_1/X_1\theta,$ $\ldots, X_i/X_i\theta, \ldots, X_n/X_n\theta](X_i) \equiv \theta(X_i) \not\equiv X_i$ by the previous fact, therefore $X_i \in \dom([X_1/X_1\theta, \ldots, X_i/X_i\theta, \ldots, X_n/X_n\theta])$, which implies $X_i \in \bigcup_{\mu \in \cc{\Theta}}\dom(\mu)$, thus $\{X_1, \ldots, X_n\} \subseteq \bigcup_{\mu \in \cc{\Theta}}\dom(\mu)$
     \item[d)] By the previous item we have that $\bigcup_{\mu \in \cc{\Theta}}\dom(\mu) = \{X_1, \ldots, X_n\}$. We will use the criterion from Lemma \ref{lemmaCompress1}, so let us take some $\mu_1, \ldots, \mu_n \in \cc{\Theta}$. By definition of $\cc{\Theta}$ we have that for each $\mu_i$ $\exists \theta_i \in \Theta$ such that $X_i\mu_i \equiv X_i\theta_i$. But then $(X_1\mu_1, \ldots, X_n\mu_n) \equiv (X_1\theta_1, \ldots, X_n\theta_n) \equiv (X_1, \ldots, X_n)[X_1/X_1\theta_1, \ldots, X_n/X_n\theta_n]$, and $[X_1/X_1\theta_1, \ldots, X_n/X_n\theta_n] \in \cc{\Theta}$ by definition of $\cc{\Theta}$, so we are done.
\end{enumerate}
\end{proof}

\begin{proof}[Proof for Lemma \ref{LemPropsCC2}]\label{PROOFLemPropsCC2}
Let $\bigcup_{\theta \in \Theta}dom(\theta) = \{X_1, \ldots, X_n\} = \bigcup_{\mu \in \cc{\Theta}}\dom(\mu)$ by Proposition \ref{LemPropsCC1}, and let us consider some $\mu \in \cc{\Theta}$. Then $\mu = [X_1/X_1\theta_1, \ldots, X_n/X_n\theta_n]$ for some $\theta_1, \ldots, \theta_n \in \Theta$. Then given some $X \in \var$ we have the following possibilities:
\begin{enumerate}
	\item[a)]$X \equiv X_i \in \{X_1, \ldots, X_n\}$: Then $\vdbp \sigma(X) \equiv \sigma(X_i) \clto \theta_i(X_i)$, as $\theta_i \in \Theta \subseteq \denbp{\sigma}$. But $X \equiv X_i \in \{X_1, \ldots, X_n\}$ implies $\theta_i(X_i) \equiv \mu(X_i) \equiv \mu(X)$, so $\vdbp \sigma(X) \clto \mu(X)$.
     \item[b)] $X \not\in \{X_1, \ldots, X_n\}$: Then we can take any $\theta_i \in \Theta$ (it must exist since $\Theta$ is not empty) so $\vdbp \sigma(X) \clto \theta_i(X_i)$, as $\theta_i \in \Theta \subseteq \denbp{\sigma}$. But then $X \not\in \dom(\theta_i)$, as $\{X_1, \ldots, X_n\} = \bigcup_{\theta \in \Theta}dom(\theta) \supseteq dom(\theta_i)$, therefore $\theta_i(X) \equiv X \equiv \mu(X)$, as $\dom(\mu) \subseteq \bigcup_{\mu \in \cc{\Theta}}\dom(\mu) = \{X_1, \ldots, X_n\}$, hence $\vdbp \sigma(X) \clto \mu(X)$.
\end{enumerate}
Thus we have proved that $\forall U \in \var, \vdbp \sigma(U) \clto \mu(U)$, henceforth $\mu \in \denbp{\sigma}$ and so $\cc{\Theta} \subseteq \denbp{\sigma}$.
\end{proof}

\begin{lemma}\label{lIcsus1}
For any $t \in \CTerm_\perp, \Theta \subseteq \CSubst_\perp$ finite, given $\theta_i \in \Theta$ then $\pps t(?\Theta) \cltop t\theta_i$.
\end{lemma}
\begin{proof}
A simple induction on the structure of $t$.
\end{proof}

%\todo{este lema se quito, la parte a) se deja inline por trivial, pero la b) creo q se usa en la demo final de correccion de un paso de term rewriting wrt \bpcrwl, reformular para q solo salga la parte b) y ponerlo donde toque}
\begin{lemma}\label{lemmaCompress2}%~
%\begin{enumerate}
%   \item[a)] For any $\theta \in CSubst_\perp$ the set $\{\theta\}$ is compressible
%	\item[b)] 
For any $\Theta \subseteq \CSubst_\perp$ compressible and ${\cal D} \subseteq \var$ we have that $\Theta' = \{\theta|_{\cal D}~|~\theta \in \Theta\}$ is also compressible.
%\end{enumerate}
\end{lemma}
\begin{proof}
%\begin{enumerate}
%   \item[a)] Trivial by the characterization of Lemma \ref{lemmaCompress1}.
%   \item[b)] 
Consider $\{Y_1, \ldots, Y_m\} = \bigcup_{\theta' \in \Theta'} \dom(\theta')$, by Lemma \ref{lemmaCompress1} all we have to prove is that $\{(Y_1\theta', \ldots, Y_m\theta')~|~\theta' \in \Theta'\} \supseteq \{Y_1\theta'~|~\theta' \in \Theta'\} \times \ldots \times \{Y_m\theta'~|~\theta' \in \Theta'\}$. To consider some element of the latter set let us fix some $\theta'_1, \ldots, \theta'_m \in \Theta'$ so we have $(Y_1\theta'_1, \ldots, Y_m\theta'_m)$. Now for $\overline{X} = \bigcup_{\theta \in \Theta} \dom(\theta)$, then by definition of $\Theta'$ we get that $\forall j \in  \{1, \ldots, m\}. \exists \theta_j \in \Theta, X_j \in \overline{X}$ such that $\theta'_j = \theta_j|_{\cal D}$ and $X_j \equiv Y_j$, so  $(Y_1\theta'_1, \ldots, Y_m\theta'_m)$ is in a sense contained in some tuple $(X_1\theta_1, \ldots, X_n\theta_n)$, as it is a subtuple of this later tuple. Then, as $\Theta$ is compressible then $\exists \theta \in \Theta$ such that $\forall j \in  \{1, \ldots, m\}. X_j\theta_j \equiv X_j\theta$, but then for each $j \in  \{1, \ldots, m\}$
$$
\begin{array}{ll}
Y_j\theta'_j \equiv X_j\theta_j|_{\cal D} & \mbox{by definition of } \Theta\\
\equiv X_j\theta_j & \mbox{ as } X_j \equiv Y_j \in {\cal D} \mbox{ by definition of } \{Y_1, \ldots, Y_m\}  \\
\equiv X_j\theta & \mbox{ taking $\theta$ above}\\
\equiv Y_j\theta & \mbox{ as } X_j \equiv Y_j\\
\equiv Y_j\theta|_{\cal D} \mbox{ as } Y_j \in {\cal D}
\end{array}
$$
But $\theta \in \Theta$ and so $\theta|_{\cal D} \in \Theta'$  by definition, and we are done as then $(Y_1\theta'_1, \ldots, Y_m\theta'_m) = (Y_1\theta|_{\cal D}, \ldots, Y_m\theta|_{\cal D}) \in \{(Y_1\theta', \ldots, Y_m\theta')~|~\theta' \in \Theta'\}$.
%\end{enumerate}
\end{proof}

\begin{proof}[Proof for Lemma \ref{LCompPlvsRw1}]\label{PROOFLCompPlvsRw1}
Let us assume the term rewriring step was performed at the root of the expression, so it has the shape $e \equiv f(\overline{p})\sigma \tor r\sigma \equiv e'$. Thus, given some $t \in \denbp{r\sigma}$ our goal is proving that $t \in \denbp{f(\overline{p})\sigma}$.  First of all by Lemma \ref{lDenSubstBPl1} we get some compressible $\Theta \subseteq \denbp{\sigma}$ such that $t \in \denbp{r(?\Theta)}$. If we could use it to prove that $t \in \denbp{f(\overline{p})(?\Theta)}$ then  by Lemma \ref{lDenSubst2} we would get $?\Theta \dsord \sigma $, so by the monotonicity of Theorem \ref{ThPropsBetaPlHeredadas} we could obtain $t \in \denbp{f(\overline{p})\sigma}$ as we wanted. 
%. The idea is that given some $t \in \denbp{r\sigma}$ then by Lemma \ref{lDenSubstBPl1} we get some compressible $\Theta \subseteq \denbp{\sigma}$ such that $t \in \denbp{r(?\Theta)}$. Our goal is proving that $t \in \denbp{f(\overline{p})\sigma}$, but by Lemmas \ref{lDenSubst2} and \ref{LMonSusPluralBEta} that is implied by $t \in \denbp{f(\overline{p})(?\Theta)}$. 
%But a
As $\overline{p} \subseteq \CTerm_\perp$ and $\Theta \subseteq \CSubst_\perp$ then by Lemma \ref{lIcsus1} we get that $\forall p_i \in \overline{p}, \theta_j \in \Theta$ we have $\vdbp p_i(?\Theta) \clto p_i\theta_j$. All this can be used to perform the following step, assuming $\Theta = \{\theta_1, \ldots, \theta_m\}$.
\begin{scriptsize}
$$
\infer[\mbox{\crule{\bpor}}]{f(p_1, \ldots, p_n)(?\Theta) \clto t}
           {
	\begin{array}{c}
        p_1(?\Theta) \cltop p_1\theta_1 \equiv p_1\theta_1|_{\mivar(p_1)} \\
	      \ \ldots \\
		p_1(?\Theta) \cltop p_1\theta_m \equiv p_1\theta_m|_{\mivar(p_1)} \\
	\end{array}~
       \ldots
       \ \begin{array}{c}
		p_n(?\Theta) \cltop p_n\theta_1 \equiv p_n\theta_1|_{\mivar(p_n)} \\
	      \ \ldots \\
		p_n(?\Theta) \cltop p_n\theta_m \equiv p_n\theta_m|_{\mivar(p_n)} \\
	\end{array}
       \ \begin{array}{c}
         ~ \\
         ~ \\
         r\theta' \equiv r(?\Theta) \cltop t
         \end{array}
            }
$$
\end{scriptsize}
for $\theta' = (\biguplus ?\Theta_i) \uplus \theta_e$ where $\forall i \in \{1, \ldots, n\}. \Theta_i = \{\theta_j|_{\mivar(p_i)}~|~\theta_j \in \Theta\}$, $\theta_e = (?\Theta)|_\vE$ for $\vE = \vextra{f(\overline{p}) \tor r}$. Note that $\forall i. \dom(?\Theta_i) \subseteq \mivar(p_i)$ by Lemma \ref{lemIntCjtoCsus}, therefore $\theta'$ is well defined by left linearity of program rules. As $\Theta$ is compressible then each $\Theta_i$ is also compressible, by Lemma \ref{lemmaCompress2}, and so they can be used to build $\theta'$ in the \bpor\ step above. All that is left is proving $r\theta' \equiv r(?\Theta)$, which holds because given any $X \in \mivar(r)$ we have $\theta'(X) \equiv (?\Theta)(X)$. As $\mivar(r) \subseteq \biguplus\limits_{i = 1}^n \mivar(p_i) \uplus \vE$ then we have two possibilities for such $X \in \mivar(r)$:
\begin{enumerate}
	\item[a)] $\exists ! p_i \in \overline{p}. X \in \mivar(p_i)$ then $\theta'(X) \equiv (?\Theta_i)(X)$. To prove that $(?\Theta_i)(X) \equiv (?\Theta)(X)$ note that as $X \in \mivar(p_i)$ then $\forall \theta_j \in \Theta$ we have that $X \in \dom(\theta_j)$ implies $X \in \dom(\theta_j)|_{var(p_i)}$, therefore $\forall \theta_j \in \Theta. X \in \dom(\theta_j)$ iff $X \in \dom(\theta_j)|_{var(p_i)}$. Now we have two possibilities:
\begin{enumerate}
	\item[i)] If $\exists \theta_j \in \Theta. X \not\in \dom(\theta_j)$ let $\rho_1 \ldots \rho_l = \theta_1 \ldots \theta_m~|~\lambda \theta.(X \in \dom(\theta))$. Then $\theta_1|_{\mivar(p_i)} \ldots \theta_m|_{\mivar(p_i)}~|~\lambda \theta.(X \in \dom(\theta)) = \rho_1|_{\mivar(p_i)} \ldots \rho_l|_{\mivar(p_i)}$ and so
$$
\begin{array}{ll}
(?\Theta)(X) \equiv X~?~\rho_1(X)~?~\ldots~?~\rho_l(X)\\
\equiv X~?~\rho_1|_{var(p_i)}(X)~?~\ldots~?~\rho_l|_{\mivar(p_i)}(X) & \mbox{ as } X \in \mivar(p_i)\\
\equiv (?\Theta_i)(X)
\end{array}
$$
    \item[ii)] Otherwise $\forall \theta_j \in \Theta. X \in \dom(\theta_j)$ and so $\forall \theta_j \in \Theta. X \in \dom(\theta_j|_{var(p_i)})$, as $X \in var(p_i)$. But then
$$
\begin{array}{ll}
(?\Theta)(X) \equiv \theta_1(X)~?~\ldots~?~\theta_m(X)\\
\equiv \theta_1|_{var(p_i)}(X)~?~\ldots~?~\theta_m|_{\mivar(p_i)}(X) & \mbox{ as } X \in \mivar(p_i)\\
\equiv (?\Theta_i)(X)
\end{array}
$$
\end{enumerate}
Therefore $\theta'(X) \equiv (?\Theta_i)(X) \equiv (?\Theta)(X)$.
    \item[b)] Otherwise $X \in \vE$, but then
$$
\begin{array}{ll}
\theta'(X) \equiv \theta_e(X) & \mbox{ by definition of $\theta'$} \\
\equiv (?\Theta)|_\vE(X) & \mbox{ by definition of $\theta_e$} \\
\equiv (?\Theta)(X) & \mbox{ as $X \in \vE$}
\end{array}
$$
\end{enumerate}

We have just proved the soundness w.r.t.\ \bpcrwl\ of term rewriting steps performed at the root of the starting expression. So all that is left is using the compositionality of \bpcrwl\ from Theorem~\ref{ThPropsBetaPlHeredadas} for propagating this result for steps performed in an arbitrary context. If the step was not performed at the root of the expression then we have $e \equiv \con[f(\overline{p})\sigma] \rw \con[r\sigma] \equiv e'$ for which $f(\overline{p})\sigma \rw r\sigma$ is performed at the top. But then $\denbp{r\sigma} \subseteq \denbp{f(\overline{p})\sigma}$ by the proof of the previous case, and we can chain:
$$
\begin{array}{ll}
\denbp{\con[r\sigma]} = \bigcup\limits_{\{t_1, \ldots, t_n\} \subseteq \denbp{r\sigma}} \denbp{\con[t_1~?~\ldots~?~t_n]} & \mbox{ by Theorem \ref{ThPropsBetaPlHeredadas}}\\
\subseteq \bigcup\limits_{\{t_1, \ldots, t_n\} \subseteq \denbp{f(\overline{p})\sigma}} \denbp{\con[t_1~?~\ldots~?~t_n]} = \denbp{\con[f(\overline{p})\sigma]} & \mbox{ by Theorem \ref{ThPropsBetaPlHeredadas}}\\
\end{array}
$$
\end{proof}

\subsection{For Section \ref{sect:equivaABPlural}}

In the proof for Theorem \ref{ThEquivABPClass} we will use the following notion of substitution modification to formalize the reduction into $\perp$ of the values that a starting matching substitution $?\Theta_i$, used in a \apor\ step, assigns to the variables in a left-hand side argument $p_i$ which are also different to the at most unique---when not absent---variable $X \in \mivar(p_i) \cap \mivar(r)$, granted because the program belongs to the class $\classAB$.


\begin{definition}[Substitution modification]\label{defSubstMod}
For any $\sigma \in \Subst_\perp$ its modification $\sigma\{X / e\} \in \Subst_\perp$, in which the value for $X \in \var$ is replaced by some $e \in \Exp_\perp$ is defined as
$$
(\sigma\{X/e\})(Y) = \left\{\begin{array}{ll}
e & \mbox{ if } X \equiv Y \\
 \sigma(Y) & \mbox{ otherwise}
\end{array}\right.
$$
\end{definition}

\begin{lemma}\label{lemAuxEquivClass1}
For any $\sigma \in \Subst_\perp$, $X \in \var$, $e \in \Exp_\perp$ we have
$$
\dom(\sigma\{X/e\}) \subseteq \dom(\sigma) \cup \{X\}
$$
\end{lemma}
\begin{proof}
Given some $Y \in \dom(\sigma\{X/e\})$, if $Y \equiv X$ then $Y \in \dom(\sigma) \cup \{X\}$. Otherwise $Y \not\equiv X$, which implies $Y \in \dom(\sigma)$ as
%$Y \in dom(\sigma\{X/e\} \setminus \{X\})$ implies $Y \not\equiv X$, and so $Y \in dom(\sigma)$, because
$$
\begin{array}{ll}
Y \not\equiv (\sigma\{X/e\})(Y) & \mbox{ as } Y \in \dom(\sigma\{X/e\}) \\
\equiv \sigma(Y) & \mbox{ as } Y \not\equiv X \\
\end{array}
$$
But then $Y \in \dom(\sigma)$ by definition.
\end{proof}

\begin{proof}[Proof for Theorem \ref{ThEquivABPClass}]\label{PROOFThEquivABPClass}
By Theorem \ref{tCrwlVsPCRWL} we just have to prove that $\denapp{e}{\prog} \subseteq \denbpp{e}{\prog}$ whenever $\prog \in \classAB$. Assume a $\apcrwl$-proof for $\prog \vdap e \clto t$ for some $e \in \Exp_\perp$, $t \in \CTerm_\perp$, we will show that we can build another $\apcrwl$-proof for the same statement which only uses compressible substitutions in \apor\ steps. As a consequence each \apor\ step will be also a valid \bpor\ step, so that will be also a $\bpcrwl$-proof for $\prog \vdbp e \clto t$.

Therefore all that is left is building the new $\apcrwl$-proof. To do that we proceed by induction on the size of the original $\apcrwl$-proof for $\prog \vdap e \clto t$, performing a case distinction over the $\apcrwl$ rule applied at the root of the starting proof. The cases for \crule{B} and \crule{RR} are trivial, and so it is the case for \crule{DC}, where we just have to apply the IH over each premise $\prog \vdap e_i \clto t_i$, then building the target $\apcrwl$-proof with an application of \crule{DC} at its root and the resulting proofs from the applications of the IH as its premises. 

The interesting case is that for an application of \apor. For the sake of simplicity we will prove if for $f \in \FS^1$, but this proof can be easily extended to functions of arbitrary arity thanks to left linearity of program rules. Then we have the following proof
$$
\infer[\mbox{\apor}]{\prog \vdap f(e) \tor t}
{
\begin{array}{l}
e \tor p\theta_1 \\
\ldots \\
e \tor p\theta_m \\
\end{array}
\begin{array}{l}
~\\ ~\\
~r\theta \clto t
\end{array}
}
$$
For some $(f(p) \tor r) \in \prog$, $\Theta = \{\theta_1, \ldots, \theta_m\}. \forall j. \dom(\theta_j) \subseteq \mivar(p)$, $\theta = ?\Theta \uplus \theta_e$ for some $\theta_e \in \icsus$. But as $\prog \in \classAB$ then we have $\#(\mivar(p) ~\cap~ \mivar(r)) = K \leq 1$. Hence either $K = 0$ or $K = 1$, let us consider both cases.

~\\
\underline{If $K = 0$}: We define $\overline{X} \subseteq \var$ as $\overline{X} = \bigcup_{j \in \{1, \ldots, m\}} \dom(\theta_j)$. Then we have $\forall j. [\overline{X/\perp}] \ordap \theta_j$ because given an arbitrary $Y \in \var$:
\begin{itemize}
	\item If $Y \in \overline{X}$ then $[\overline{X/\perp}](Y) \equiv \perp \ordap \theta_j(Y)$.
	\item Otherwise $Y \not\in \overline{X}$. But $\dom(\theta_j) \subseteq \overline{X}$ by definition of $\overline{X}$, and so $Y \not\in \dom(\theta_j)$, hence $[\overline{X/\perp}](Y) \equiv Y \ordap Y \equiv \theta_j(Y)$. 
\end{itemize}
Then we can take an arbitrary $\theta_j \in \{\theta_1, \ldots, \theta_m\}$ for which $[\overline{X/\perp}] \ordap \theta_j$ implies $p[\overline{X/\perp}] \ordap p\theta_j$ (easy to check by induction on the structure of expressions). But then applying the polarity of \apcrwl\ from Proposition \ref{LMonPlural} over the statement $e \clto p\theta_j$ we get $e \clto p[\overline{X/\perp}]$ with a proof of the same size or smaller. Hence we can apply the IH over $e \clto p[\overline{X/\perp}]$ and $r\theta \clto t$ to get a \apcrwl-proof for both statements in which only compressible substitutions are used. 

All that is left is proving that by reducing $e$ to $p[\overline{X/\perp}]$ we can build a substitution $\theta'$ with the same effect over $r$ as $\theta$, using a compressible substitutions in the \apor\ step also. First of all, as $K = 0$ then $\mivar(p) ~\cap~ \mivar(r) = \emptyset$. Besides, as $\forall j. \dom(\theta_j) \subseteq \mivar(p)$ by hypothesis, then $\overline{X} \subseteq \mivar(p)$ by definition, and so $\overline{X} \cap \mivar(r) = \emptyset$. Furthermore, by Lemma \ref{lemIntCjtoCsus} we have $\dom(?\Theta) = \bigcup_{j \in \{1, \ldots, m\}} \dom(\theta_j) = \overline{X}$, hence $\dom(?\Theta) \cap \mivar(r) = \emptyset$. But then if we define $\theta' = ?\{[\overline{X/\perp}]\} \uplus \theta_e = [\overline{X/\perp}] \uplus \theta_e$ then we can chain
$$
\begin{array}{ll}
r\theta' \equiv r([\overline{X/\perp}] \uplus \theta_e) \\
\equiv r\theta_e & \mbox{ as } \overline{X} \cap var(r) = \emptyset \\
\equiv r(?\Theta \uplus \theta_e) & \mbox{ as } \dom(?\Theta) \cap \mivar(r) = \emptyset\\
\equiv r\theta
\end{array}
$$
Besides, the set $\{[\overline{X/\perp}]\}$ is compressible because it is singleton---trivial by the characterization of Lemma \ref{lemmaCompress1}. So we can finally take the \apcrwl-proofs obtained by IH to build the following \apcrwl-proof that only uses compressible substitutions.
$$
\infer[\mbox{\apor}]{\prog \vdap f(e) \clto t}
{
e \clto p[\overline{X/\perp}]
~~~~ r\theta' \equiv r\theta \clto t
}
$$

~\\
\underline{If $K = 1$}: Let us define $\overline{X} = \bigcup_{j \in \{1, \ldots, m\}} \dom(\theta_j)$, for which $\overline{X} \subseteq \mivar(p)$ like in the previous case. As $K = 1$ then $\exists ! Y \in \var. \mivar(p) \cap \mivar(r) = \{Y\}$. Then we have $\forall j. [\overline{X/\perp}]\{Y/\theta_j(Y)\} \ordap \theta_j$, because given an arbitrary $Z \in \var$:
\begin{itemize}
	\item If $Z \equiv Y$ then $([\overline{X/\perp}]\{Y/\theta_j(Y)\})(Z) \equiv \theta_j(Y) \ordap \theta_j(Y) \equiv \theta_j(Z)$. 
    \item If $Z \in \overline{X} \setminus \{Y\}$ then $([\overline{X/\perp}]\{Y/\theta_j(Y)\})(Z) \equiv [\overline{X/\perp}](Z) \equiv \perp \ordap \theta_j(Z)$. 
    \item Otherwise $Z \not\equiv Y$ and $Z \not\in \overline{X}$, which implies $Z \not\in dom(\theta_j)$ by definition of $\overline{X}$, but then $([\overline{X/\perp}]\{Y/\theta_j(Y)\})(Z) \equiv [\overline{X/\perp}](Z) \equiv Z \ordap Z \equiv \theta_j(Z)$. 
\end{itemize}
Then $\forall \theta_j \in \{\theta_1, \ldots \theta_m\}$ we have $p[\overline{X/\perp}]\{Y/\theta_j(Y)\} \ordap p\theta_j$ and we can apply the polarity of \apcrwl\ from Proposition \ref{LMonPlural} over each statement $e \clto p\theta_j$ to get $e \clto p[\overline{X/\perp}]\{Y/\theta_j(Y)\}$ with a proof of the same size or smaller. Hence we can apply the IH over each of that proofs and over the proof for $r\theta \clto t$ to get \apcrwl-proofs for each of those statements in which only compressible substitutions are used. 

All that is left is proving that by reducing $e$ to those values we can build a substitution $\theta'$  with the same effect over $r$ as $\theta$, but also using a compressible substitution in the \apor\ step. This substitution will be 
$$
\Theta' = \{[\overline{X/\perp}]\{Y/\theta_j(Y)\}~|~\theta_j \in \{\theta_1, \ldots, \theta_m\}\}
$$

Regarding the first part, as $\overline{X} \subseteq \mivar(p)$ then $\dom([\overline{X/\perp}]) \subseteq \mivar(p)$. Besides, by Lemma \ref{lemAuxEquivClass1} we get $\forall \theta_j. \dom([\overline{X/\perp}]\{Y/\theta_j(Y)\}) \subseteq \dom([\overline{X/\perp}]) \cup \{Y\}$, which combined with the previous fact yields $\forall \theta_j.\dom([\overline{X/\perp}]$ $\{\theta_j(Y)\}) \subseteq \mivar(p) \cup \{Y\}$. Then combining this with Lemma \ref{lemIntCjtoCsus} we get $\dom(?\Theta') = \bigcup_{\theta_j}\dom([\overline{X/\perp}]$ $\{Y/\theta_j(Y)\}) \subseteq \mivar(p) \cup \{Y\}$. But as $\mivar(p) \cap \mivar(r) = \{Y\}$ then $\dom(?\Theta') \cap \mivar(r) \subseteq \{Y\}$. Similarly we can prove $\dom(?\Theta) \cap \mivar(r) \subseteq \{Y\}$, because $\forall \theta_j. \dom(\theta_j) \subseteq \mivar(p)$, which implies $\dom(?\Theta) \subseteq \mivar(p)$ by Lemma \ref{lemIntCjtoCsus}. But then if we define $\theta' = ?\Theta' \uplus \theta_e$ then we can chain
$$
\begin{array}{ll}
r\theta \equiv r(?\Theta \uplus \theta_e) \\
\equiv r((?\Theta)|_{\{Y\}} \uplus \theta_e) & \mbox{ as } \dom(?\Theta) \cap \mivar(r) \subseteq \{Y\} \\
\equiv r([Y/(?\Theta)(Y)] \uplus \theta_e) \\
\equiv r([Y/(?\Theta')(Y)] \uplus \theta_e) & (*)\\
\equiv r((?\Theta')|_{\{Y\}} \uplus \theta_e) & \mbox{ as } \dom(?\Theta') \cap \mivar(r) \subseteq \{Y\} \\
\equiv r(?\Theta' \uplus \theta_e) \equiv r\theta'\\
\end{array}
$$
$(*)$ as $(?\Theta)(Y) \equiv (?\Theta')(Y)$, because $\forall \theta_j. ([\overline{X/\perp}]\{Y/\theta_j(Y)\})(Y) \equiv \theta_j(Y)$, therefore $\forall \theta_j. Y \in \dom([\overline{X/\perp}]\{Y/\theta_j(Y)\})$ iff $Y \in \dom(\theta_j)$, which implies that given $\rho_1 \ldots \rho_l = \theta_1  \ldots \theta_m~|~\lambda \theta. (Y \in \dom(\theta))$ then $[\overline{X/\perp}]\{Y/\theta_1(Y)\} \ldots [\overline{X/\perp}]\{Y/\theta_m(Y)\}$ $|~\lambda \theta. (Y \in \dom(\theta)) = [\overline{X/\perp}]\{Y/\rho_1(Y)\} \ldots [\overline{X/\perp}]\{Y/\rho_l(Y)\}$. But then we have two possibilities:
\begin{enumerate}
	\item If $\exists \theta_j. Y \not\in \dom(\theta_j)$ then $Y \not\in \dom([\overline{X/\perp}]\{Y/\theta_j(Y)\})$, therefore
$$
\begin{array}{ll}
(?\Theta)(Y) \equiv Y~?~\rho_1(Y)~?~\ldots~\rho_l(Y) \\
\equiv Y~?~([\overline{X/\perp}]\{Y/\rho_1(Y)\})(Y)~?~\ldots~([\overline{X/\perp}]\{Y/\rho_l(Y)\})(Y) \\
\equiv (?\Theta')(Y)
\end{array}
$$
    \item Otherwise $\forall \theta_j. Y \in \dom(\theta_j)$, thus $\forall \theta_j. Y \in \dom([\overline{X/\perp}]\{Y/\theta_j(Y)\})$, therefore
$$
\begin{array}{ll}
(?\Theta)(Y) \equiv \theta_1(Y)~?~\ldots~\theta_m(Y) \\
\equiv ([\overline{X/\perp}]\{Y/\theta_1(Y)\})(Y)~?~\ldots~([\overline{X/\perp}]\{Y/\theta_m(Y)\})(Y) \\
\equiv (?\Theta')(Y)
\end{array}
$$
\end{enumerate}
We will now use the characterization of Lemma \ref{lemmaCompress1} to prove that $\Theta'$ is compressible. Let us define $\overline{U} = \{U_1, \ldots, U_k\} = \bigcup_{\theta' \in \Theta'} \dom(\theta')$. By definition of $\Theta'$ each $\theta'_j$ is of the form $\theta'_j = [\overline{X/\perp}]\{Y/\theta_j(Y)\}$. Now we have two possibilities:
\begin{enumerate}
	\item If $Y \in \overline{U}$ then $Y \equiv U_l$ for some $U_l \in \overline{U}$. By Lemma \ref{lemmaCompress1} we can prove that $\Theta'$ is compressible if we can find some $\theta'  \in \Theta'$ such that $\forall j \in \{1, \ldots, k\}. U_j\theta' \equiv U_j\theta'_j$. We can take $\theta' = \theta'_l$, for which given an arbitrary $U_j \in \overline{U}$:
\begin{enumerate}
	\item If $j = l$ then $U_j\theta' \equiv U_l\theta'_l \equiv U_j\theta'_j$.
    \item Otherwise $j \neq l$, but then
$$
\begin{array}{ll}
U_j\theta'_j \equiv U_j([\overline{X/\perp}]\{Y/\theta_j(Y)\}) \\
\equiv U_j[\overline{X/\perp}] & \mbox{ as $j \neq l$, which implies $U_j \not\equiv U_l \equiv Y$}\\
\equiv U_j([\overline{X/\perp}]\{Y/\theta_l(Y)\}) & \mbox{ as  $U_j \not\equiv Y$}\\
\equiv U_j\theta'_l \equiv U_j\theta'
\end{array}
$$
\end{enumerate}
    \item Otherwise $Y \not\in \overline{U}$, and then we can take $\theta' = \theta'_j$ for some arbitrary $\theta'_j \in \Theta'$, and proceed like in the second item of the previous case. 
\end{enumerate}

Now, we can finally take the \apcrwl-proofs obtained by IH to build the following \apcrwl-proof that only uses compressible substitutions.
$$
\infer[\mbox{\apor}]{\prog \vdap f(e) \clto t}
{
\begin{array}{l}
e \clto [\overline{X/\perp}]\{Y/\theta_1(Y)\} \\
\ldots \\
e \clto [\overline{X/\perp}]\{Y/\theta_m(Y)\} \\
\end{array}
~~~~ \begin{array}{l}
~ \\ ~ \\ r\theta' \equiv r\theta \clto t \\
\end{array}
}
$$
\end{proof}


\subsection{For Section \ref{sec:simulAPlural}}
We will use the following simple auxiliary lemma for proving Theorem \ref{TPstSound}. 
\begin{lemma}\label{LAuxTPstSound2}
For any \crwl-program $\prog$ and any \pcrwl-statement $\mi{if}~e_1~\thn~e_2 \cltop t$ there is a \pcrwl-proof for that statement of the form:
$$
\infer[\crule{POR}]{\mi{if}~e_1~\mi{then}~e_2 \cltop t}
           {
           e_1 \cltop \tru~
         & e_2 \cltop t~
         & t \cltop t
           }
$$
\end{lemma}
\begin{proof}
As the only rule for $\mi{if}\_\mi{then}\_$ is $\mi{if}~\tru~\mi{then}~X \tor X$ then every proof must be of the form:
$$
\infer[\crule{POR}]{\mi{if}~e_1~\mi{then}~e_2 \cltop t}
           {
           \begin{array}{l}
            e_1 \cltop \tru\theta_1 \\ \ldots \\ e_1 \cltop \tru\theta_m 
           \end{array}~
\           \begin{array}{l}
           e_2 \cltop t_1 \\ \ldots \\ e_2 \cltop t_l 
           \end{array}~
         \ t_1?\ldots?t_l \cltop t
           }
$$
As $t_1~?~\ldots~?~t_l \cltop t$ there must exist some $t_i \in \{t_1, \ldots, t_l\}$ such that $t_i \cltop t$, but then $t \ordap t_i$ by Lemma \ref{lSimplePropPCRWL} and so $e_2 \cltop t_i$ implies $e_2 \cltop t$ by Proposition \ref{LMonPlural}, and we can apply Lemma \ref{lSimplePropPCRWL} again to get $t \cltop t$ and construct the proof of the formulation.
% And it is clear that taking $t \equiv t_i$ the proof of the formulation is also a proof for $if~e_1~then~e_2 \cltop t$.
% But as $\tru$ is ground then every $\theta_j$ must be equal to $\epsilon$, so every $e_1 \cltop \tru\theta_1 \equiv  e_1 \cltop \tru$, which is the only proof needed for the first argument. Besides if $t_1?\ldots?t_l \cltop t$ then 
\end{proof}

Now we are ready to prove Theorem \ref{TPstSound}. 

\begin{proof}[Proof for Theorem \ref{TPstSound}]\label{PROOFTPstSound}
As seen in Section \ref{sec:simulAPlural}, the second part follows from combining the first part with Corollary \ref{CHierChain}, because then we can chain $\denrp{e}{\pst{\prog}} \subseteq \denapp{e}{\pst{\prog}} \subseteq \denapp{e}{\prog}$.\\

So all that is left is proving the first part. Let us assume $\pst{\prog} \pps e \cltop t$ for some $t \in \CTerm_\perp$, we will see that then ${\prog} \pps e \cltop t$ by induction on the size of $\pst{\prog} \pps e \cltop t$. The base cases are trivial because no program rule is involved, and so it is the case for \crule{DC}, in which we only have to apply the IH over the hypothesis. The case for \apor\ when $e \equiv f(\overline{e})$ and $f \in \{\_?\_, \mi{if}\_\mi{then}\_\}$ can be resolved applying the IH too, so the difficult case is that in which $f \not\in \{\_?\_, \mi{if}\_\mi{then}\_\}$. For the sake of simplicity we will consider $f \in \FS^1$, the proof can be easily extended to functions with zero or more than one arguments. Assume the rule used was $f(Y) \tor \mi{if}~\match(Y)~\thn~r[\overline{X_j/\prj_j(Y)}]$, corresponding to the original rule $f(p) \tor r$ and with the auxiliary functions defined by $\match(p) \tor \tru$, $\prj_j(p) \tor X_j$, for $\overline{X_j} = \mi{var}(p) \cap \mi{var}(r)$. Then the proof has the shape:
$$
\infer[\mbox{\apor}]{\pst{\prog} \pps f(e) \cltop t}
           {\begin{array}{l}
            e \cltop t_1 \\
           \ldots \\
           e \cltop t_m
            \end{array}
   \       \begin{array}{l}~\\~\\\mi{if}~\match(t_1?\ldots?t_m)~\thn~r[\overline{X_j/\prj_j(t_1?\ldots?t_m)}] \cltop t\end{array}
            }
$$
where
\begin{footnotesize}$$
\infer[\mbox{\apor}]{\pst{\prog} \pps \mi{if}~\match(t_1?\ldots?t_m)~\thn~r[\overline{X_j/\prj_j(t_1?\ldots?t_m)}] \cltop t}
          {
            \infer[\mbox{\apor}]{\match(t_1?\ldots?t_m) \cltop \tru}
                       {
                       t_1?\ldots?t_m \cltop p\mu~
                    \ \tru \cltop \tru
                        }
         & r[\overline{X_j/\prj_j(t_1?\ldots?t_m)}] \cltop t
         & t \cltop t
           }
$$
\end{footnotesize}by Lemma \ref{LAuxTPstSound2}. 
Let $s_1 \ldots s_l = t_1 \ldots t_m~|~\lambda t.(\exists \theta \in \CSubst_\perp. t \equiv p\theta \ \wedge\ \dom(\theta) \subseteq \mivar(p))$. % with $dom(\theta) = var(p)$, for some $\theta \in CSubst_\perp$, one $\theta$ for each $s$ in $s_1 \ldots s_n$. 
These $s_1 \ldots s_l$ are the useful values computed for $e$ in the starting \apcrwl-proof, that is, those that can be proyected later. We will use those $\theta_j$ corresponding to each $s_j$ soon. 

Now we will see that $s_1 \ldots s_l$ is not empty. As $\pst{\prog} \pps t_1~?~\ldots~?~t_m \cltop p\mu$ then $\exists j \in \{1, \ldots, m\}$ such that $\pst{\prog} \pps t_j \cltop p\mu$, and so $p\mu \ordap t_j$ by Lemma \ref{lSimplePropPCRWL}. But then it is easy to prove by induction on the structure of $p$, taking advantage of its linearity and totality, that there must exist some $\theta_j \in \CSubst_\perp$ such that $t_j \equiv p\theta_j$. 
%
Hence $s_1 \ldots s_l$ is not empty and then 
it is easy to prove that $[\overline{X_j/\prj_j(t_1?\ldots?t_m)}]$ and $[\overline{X_j/\prj_j(s_1?\ldots?s_l)}]$ verify the conditions to apply the strong monotonicity of Proposition \ref{LMonSusPlural} in order to get that $\pst{\prog} \pps r[\overline{X_j/\prj_j(s_1?\ldots?s_l)}] \cltop t$ with a proof of the same size or smaller. By definition $s_1 \ldots s_l \equiv p\theta_1 \ldots p\theta_l$, now we will see that the substitutions $[\overline{X_j/\prj_j(s_1?\ldots?s_l)}]$ and $?\{\theta_1, \ldots, \theta_l\}|_{\mivar(r)}$ also verify the conditions of to apply the strong monotonicity of Proposition \ref{LMonSusPlural}. As $\forall \theta \in \{\theta_1, \ldots, \theta_l\}. \dom(\theta) \subseteq \mivar(p)$ then $\dom(?\{\theta_1, \ldots, \theta_l\}|_{\mivar(r)}) \subseteq \overline{X_j}$, so given $X \not\in \overline{X_j}$ both substitutions leave it untouched. On the other hand if $X \equiv X_j \in \overline{X_j}$, given
$$
\scalebox{.93}{
\infer[\mbox{\apor}]{\pst{\prog} \pps X_j[\overline{X_j/\prj_j(s_1~?~\ldots~?~s_l)}] \equiv \prj_j(s_1~?~\ldots~?~s_l) \cltop t}
           {
           \begin{array}{l}
            s_1~?~\ldots~?~s_l \cltop p\mu_1 \\ \ldots \\ s_1~?~\ldots~?~s_l \cltop p\mu_h
           \end{array}~
         \ \begin{array}{l}~\\~\\X_j(?\{\mu_1, \ldots, \mu_h\}) \cltop t\end{array}
            }
}
$$
Then $\pst{\prog} \pps X_j(?\{\mu_1, \ldots, \mu_h\}) \cltop t$ implies that $\pst{\prog} \pps \mu(X_j) \cltop t$ for some $\mu \in \{\mu_1, \ldots, \mu_h\}$. But then $\pst{\prog} \pps s_1?\ldots?s_l \cltop p\mu$, and so $\pst{\prog} \pps s \cltop p\mu$ for some $s \in \{s_1, \ldots, s_l\}$. Hence, by Lemma \ref{lSimplePropPCRWL} $t \ordap \mu(X_j)$ and $p\mu \ordap s$, and as $s_1 \ldots s_l \equiv p\theta_1 \ldots p\theta_l$ by definition then $p\mu \ordap s \equiv p\theta$ for some $\theta \in \{\theta_1, \ldots, \theta_l\}$. But as $X_j \in \overline{X_j} \subseteq \mivar(p)$ then $p\mu \ordap p\theta$ implies $\mu(X_j) \ordap \theta(X_j)$, hence $t \ordap \mu(X_j) \ordap \theta(X_j)$ and $\pst{\prog} \pps \theta(X_j) \cltop t$ with a proof of the same size or smaller, by Proposition \ref{LMonPlural}, and so $\pst{\prog} \pps X_j(?\{\theta_1, \ldots, \theta_l\}|_{\mivar(r)}) \cltop t$ with a proof of the same size or smaller than the proof for $\pst{\prog} \pps X_j[\overline{X_j/\prj_j(s_1?\ldots?s_l)}] \cltop t$. But then we can apply Proposition \ref{LMonSusPlural} to get $\pst{\prog} \pps r(?\{\theta_1, \ldots, \theta_l\}|_{\mivar(r)}) \cltop t$ to which we can apply the IH to get ${\prog} \pps r(?\{\theta_1, \ldots, \theta_l\}|_{\mivar(r)}) \cltop t$. We can also apply the IH to each $\pst{\prog} \pps e \cltop t_i \equiv s_l \equiv p\theta_l$ (by definition of $s_1 \ldots s_l$ there must exists some $t_i$ corresponding to each $s_l$) and build the following proof:
$$
\infer[\mbox{\apor}]{\prog \pps f(e) \cltop t}
           {
          \begin{array}{l}
           e \cltop s_1 \equiv p\theta_1 \\ \ldots \\ e \cltop s_l \equiv p\theta_l
          \end{array}~
          ~\begin{array}{l}~\\~\\ r(?\{\theta_1, \ldots, \theta_l\}) \equiv r(?\{\theta_1, \ldots, \theta_l\}|_{\mivar(r)})
            \cltop t
           \end{array}
            }
$$
\end{proof}

\begin{lemma}\label{lAuxCompPstAlt}
For every $e \in \Exp$ and $p \in \CTerm$ linear, given $\theta \in \CSubst_{\perp}$ such that $\dom(\theta) \subseteq \mi{FV}(p)$, if $p\theta \ordap |e|$ then $\exists \sigma \in \Subst$ such that $\dom(\sigma) = \dom(\theta)$, $p\sigma \equiv e$ and $\theta \ordap \sigma$.
\end{lemma}
\begin{proof}
%See \cite{LRStchrRTCT08long}. \todo{debe de ser una induccion chorra, ver la cita de arriba y sketechear la estructura aqui}
By induction on the structure of $p\theta$:
\begin{description}
 \item[Base cases]~
\begin{itemize}
 \item $p\theta \equiv Y \in \var$ : %Then $p \equiv X \in \var$ and $p\theta \equiv Y \ordap |e|$ implies $Y \equiv |e|$ and so $Y \equiv e$. But then we can take $\sigma = \theta$ to get $p\sigma \equiv p\theta \equiv Y \equiv e$, and $\theta \ordap \sigma$ as $\sigma \ordap \sigma$.
Then $p\theta \equiv Y \ordap |e|$ implies $Y \equiv |e|$ and so $Y \equiv e$. But then we can take $\sigma = \theta$ to get $p\sigma \equiv p\theta \equiv Y \equiv e$, $\theta \ordap \sigma$ as $\sigma \ordap \sigma$, and $\dom(\sigma) = \dom(\theta)$.% \subseteq FV(p)$.

 \item $p\theta \equiv c \in \CS^0$ : Then $p\theta \equiv c \ordap |e|$ implies $c \equiv |e|$ and so $c \equiv e$. But then we can take $\sigma = \theta$ to get $p\sigma \equiv p\theta \equiv c \equiv e$, $\theta \ordap \sigma$ as $\sigma \ordap \sigma$, and $\dom(\sigma) = \dom(\theta)$.% \subseteq FV(p)$.

 \item $p\theta \equiv \perp$ : Then $p \equiv X \in \var$, and $\theta = [X/\perp]$, as $\dom(\theta) \subseteq \mi{FV}(p) = \{X\}$. But then we can choose $\sigma = [X/e]$ to get $p\sigma \equiv X[X/e] \equiv e$, $\theta = [X/\perp] \ordap [X/e] \equiv \sigma$, and $\dom(\sigma) = \{X\} = \dom(\theta)$.%FV(p)$.
\end{itemize}

 \item[Inductive steps]~
\begin{itemize}
 \item $p\theta \equiv c(s_1, \ldots, s_n)$ with $p \equiv X \in \var$ : %Then $p\theta \equiv c(s_1, \ldots, s_n) \ordap |e|$ implies $|e| \equiv c(|e_1|, \ldots, |e_n|)$ and $e \equiv c(e_1, \ldots, e_n)$ such that $\forall i, s_i \ordap |e_i|$
Then $\dom(\theta) \subseteq \mi{FV}(p)$ implies $\dom(\theta) = \{X\}$, so $\theta = [X/X\theta] = [X/p\theta]$. As $\theta \in \CSubst_{\perp}, p \in \CTerm$ then $p\theta \in \CTerm_{\perp}$ and so $p\theta \ordap |e|$ implies $p\theta \ordap e$ by \textit{b)}%lemma \ref{lAuxComp2}
. But then we can choose $\sigma = [X/e]$ to get $p\sigma \equiv X[X/e] \equiv e$, $\theta = [X/p\theta] \ordap [X/e] \equiv \sigma$, and $\dom(\sigma) = \{X\} = \dom(\theta)$.%FV(p)$.

 \item $p\theta \equiv c(p_1\theta, \ldots, p_n\theta)$ with $p \equiv c(p_1,
   \ldots, p_n)$. Then $p\theta \equiv c(p_1\theta, \ldots, p_n\theta) \ordap
   |e|$ implies $|e| \equiv c(|e_1|, \ldots,$ $|e_n|)$ for $e \equiv c(e_1,
   \ldots, e_n)$ such that $\forall i,~p_i\theta \ordap |e_i|$. As $p$ is linear
   and $\dom(\theta) \subseteq \mi{FV}(p)$ then if for every $i$ we define $\theta_i =
   \theta|_{\mi{FV}(p_i)}$ then $\theta = \theta_1 \uplus \ldots \uplus
   \theta_n$. But then for every $i$ we have $p_i\theta_i \ordap |e_i|$ to which
   we can apply the IH to get  $\exists \sigma_i \in \Subst$ such that
   $p_i\sigma_i \equiv e_i$, $\theta_i \ordap \sigma_i$ and $\dom(\sigma_i) =
   \dom(\theta_i)$. But as $p$ is linear then $\sigma = \sigma_1 \uplus \ldots
   \uplus \sigma_n$ is correctly defined and $p\sigma \equiv c(p_1\sigma_1,
   \ldots, p_n\sigma_n) \equiv c(e_1, \ldots, e_n) \equiv e$, $\theta \ordap
   \sigma$ and $\dom(\sigma) = \dom(\sigma_1) \cup \ldots \cup \dom(\sigma_n) =
   \dom(\theta_1) \cup \ldots \cup \dom(\theta_n) = \dom(\theta)$.
%$\exists \sigma_i \in Subst$ such that $p_i\sigma_i \equiv e_i$, $\theta_i \ordap \sigma_i$ and $dom(\sigma_i) \subseteq FV(p_i)$. But as $p$ is linear then $\sigma = \sigma_1 \uplus \ldots \uplus \sigma_n$ is correctly defined and $p\sigma \equiv c(p_1\sigma_1, \ldots, p_n\sigma_n) \equiv c(e_1, \ldots, e_n) \equiv e$, $\theta \ordap \sigma$ and $dom(\sigma) = dom(\sigma_1) \cup \ldots \cup dom(\sigma_n) \subseteq FV(p_1) \cup \ldots \cup FV(p_n) = FV(p)$.
\end{itemize}
\end{description}

\end{proof}

A typical approach for proving Lemma \ref{lAuxCompPstAlt2} would proceed by induction on the %structure or the 
size of the starting \apcrwl-proof $\prog \uplus \progm \pps e \cltop t$ of the hypothesis. Unfortunately it does not work, as we can see considering the case %where the starting 
for the expression %is
$f(e)$ with $f \in \FS^{\prog}$, and the following starting \apcrwl-proof, using a program rule $(f(p) \tor r) \in \prog$.
$$
\infer[\mbox{\apor}]{\prog \uplus \progm \vdap f(e) \clto t}
{
\begin{array}{l}
e \clto p\theta_1 \\ \ldots \\ e \clto p\theta_m
\end{array}
~~
\begin{array}{l}
~ \\ ~ \\ r?\{\theta_1, \ldots, \theta_m\} \clto t
\end{array}
}
$$
The transformed rule corresponding to $(f(p) \tor r)$ would be  $f(Y) \tor \mi{if}~\match(Y)$ $\thn~r[\overline{X_i/\prj_i(Y)}]$, where $\overline{X_i} = var(p) \cap var(r)$, % = var(r)$ (as $var(r) \subseteq var(p)$, because we have no extra variables in program rules),
while the rules for $\match$ and each $\prj_i$ would be $\match(p) \tor \tru$, $\prj_i(p) \tor X_i$. 

We could then choose an arbitrary $\theta_j \in \{\theta_1, \ldots, \theta_m\}$ and apply the induction hypothesis over its corresponding \apcrwl-proof $\prog \uplus \progm \vdap e \clto p\theta_j$, thus getting $\progh \uplus \progm \vdash e \rw^* e'_j$ such that $p\theta_j \ordap |e'_j|$. Then, as $p$ is linear because it is in the left-hand side of a program rule, %it is easy to prove---see Lemma \ref{lAuxCompPstAlt} in \ref{proofs}---
by Lemma \ref{lAuxCompPstAlt} 
%that 
there must exists some $\sigma_j \in Subst$ such that $p\sigma_j \equiv e'_j$, so we can do
$$
\begin{array}{l}
\progh \uplus \progm \vdash f(e) \rw \mi{if}~\match(e)~\thn~r[\overline{X_i/\prj_i(e)}] \\
\rw^* \mi{if}~\match(e'_j)~\thn~r[\overline{X_i/\prj_i(e)}] \\
\equiv \mi{if}~\match(p\sigma_j)~\thn~r[\overline{X_i/\prj_i(e)}] \\
\rw \mi{if}~\tru~\thn~r[\overline{X_i/\prj_i(e)}] \rw r[\overline{X_i/\prj_i(e)}] 
\end{array}
$$
The problem now is that we must find a way to apply the induction hypothesis over $\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \clto t$. Although we can in fact prove that this statement holds, as we will see later, the corresponding \apcrwl-proof cannot be granted to have in general a smaller or equal size than the proof for $\prog \uplus \progm \vdap r?\{\theta_1, \ldots, \theta_m\} \clto t$, as the computation for each $e \clto p\theta_j$ statement might have been replicated several times in the proof for $r[\overline{X_i/\prj_i(e)}] \clto t$ because of the copies of $e$ performed by the parameter passing substitution for the term rewriting step $f(e) \rw \mi{if}~\match(e)~\thn~r[\overline{X_i/\prj_i(e)}]$. Besides, another extra work is caused by the evaluation of the calls to each $\prj_i$ function, that does not have to be performed in $r?\{\theta_1, \ldots, \theta_m\} \clto t$. 

This can be seen for example in the sample use of the transformation at the beginning of %this subsection
Section \ref{subsect:simpletrans}, where the first term rewriting step makes several copies of $c(0)~?~c(1)$. There $r?\{\theta_1, \ldots, \theta_m\}$ would be $d(0~?~1, 0~?~1)$ and $r[\overline{X_i/\prj_i(e)}]$ would be $d(\prj(c(0)~?~c(1)), \prj(c(0)~?~c(1)))$: although it is clear that both expressions can be reduced by \apcrwl\ to e.g., the value $d(0,1)$, it is also clear that the \apcrwl-proof for the latter expression will be bigger than the one for the former. 

~\\ 
The conclusion then is that we must look for another well-founded relation upon our inductive proof could be based on. To do that we must first introduce the following notions, %.
which allow us to talk more directly about the building blocks of \apcrwl-proofs.
\begin{definition}
Given a \pcrwl-proof $\pru$ for a \pcrwl-statement $e \cltop t$.
\begin{itemize}
    \item $\prem{\pru}$ denotes the multiset of \pcrwl-statements that compose $\pru$, including $e \cltop t$. We will sometimes use $\prem{e \cltop t}$ when $\pru$ is implicit.
    \item $\uprem$ is the metavariable we will use to refer to a \pcrwl-statement.
    \item $\pruD{\uprem}$ refers to the subproof for some premise $\uprem$ of $\pru$, when $\pru$ is implicit.
\end{itemize}
\end{definition}

%These notions allow us to talk more directly about the building blocks of \apcrwl-proofs. We will use them 
We can now use these notions 
to define the well-founded relation we are looking for.
\begin{definition}
For any proof $\pru$ for $\prog \uplus \progm \pps e \cltop t$ we define $\sA{\pruD{e \cltop t}}$---statements after $\prog$---as:
$$
\sA{\pruD{e \cltop t}} = \{e' \cltop t' \mid (e' \cltop t') \in \prem{e \cltop t} \wedge e' \equiv f(\overline{a})\mbox{ for some } f \in \FS^\prog \}
% ((e\equiv e' \wedge t' \equiv t) \vee e' \cltop t) \}
$$
Note that $\sA{e \cltop t}$ is a set, not a multiset. %Besides for any $\uprem \in \prem{e \cltop t}$ we have $\sA{\uprem} \subseteq \sA{e \cltop t}$ by definition. 
For any \pcrwl-proof $\pru$ by $\size{\pru}$ we denote the number of rules of the calculus used.

\noindent We define the relation $\ordLex$ over pairs of \pcrwl-proofs $\pru_1, \pru_2$, by 
$$
\pru_1 \ordLex \pru_2 \mbox{ iff } 
~~\begin{array}{c}
\sA{\pru_1} \subset \sA{\pru_2} \\
\mbox{ or } \\
\sA{\pru_1} = \sA{\pru_2} \mbox{ and } \size{\pru_1} < \size{\pru_2}
\end{array}
$$
\end{definition}

For the relation $\ordLex$ to be useful in inductions it must be well-founded, the subject of the following result.
\begin{lemma}
For any program $\prog \uplus \progm$ the relation $\ordLex$ over pairs of \pcrwl-proofs is well-founded. 
\end{lemma}
\begin{proof}
It is enough to prove that there is no infinite descending chain $\ldots \ordLex \pru_3 \ordLex \pru_2 \ordLex \pru_1$ \cite{baader-nipkow}. And this chain does not exists because \apcrwl-proofs are finite and therefore for any proof $\pru$ we have that $\sA{\pru}$ is finite---thus there are finitely many proper subsets of it---and $\size{\pru}$ is a natural number.
\end{proof}

%We will in fact 
Now we will prove Lemma \ref{lAuxCompPstAlt2} by induction over $\ordLex$ applied to $\prog \uplus \progm \pps e \cltop t$. To do that we %will use the following auxiliary but interesting results. 
still need some auxiliary results. 
% 
%\todo{este lema creo que deberia caerse para el apendice si al final no se usa en el sketch}
Next result is pretty technical, but just states the existence of a class of \apcrwl-proofs that do not have useless loops inside. 
\begin{lemma}\label{lAuxCompPstAlt3}
For any \pcrwl-statement $e \cltop t$ which holds exists some \pcrwl-proof $\pru$ such that $\forall e' \cltop t' \in \prem{\pru}$, $e' \cltop t'$ is not a premise, neither directly nor indirectly, of itself in $\pru$.
\end{lemma}
\begin{proof}
As $e \cltop t$ holds we may assume some \pcrwl-proof $\pru$ for it. If no $e' \cltop t' \in \prem{\pru}$ is premise of itself then we are done. Otherwise as any \pcrwl-proof is finite then taking the subproof corresponding to some $e' \cltop t'$ which is premise of itself there must be some $e' \cltop t'$ which does not have $e' \cltop t'$ as its premise in its corresponding proof. Then we can use that proof to replace the subproof for $e' \cltop t'$, as the proof is finite this process ends, because each time the number of sentences premises of itself decreases.
\end{proof}
%
The following result shows how $\ordLex$ in some sense extends the principle of induction over the structure of a \apcrwl-proof.
\begin{lemma}\label{lemOrdLexExtStruct}
Under any program $\prog \uplus \progm$, for any a proof $\pru$ for $\prog \uplus \progm \vdap e \clto t$ %which fulfils the conditions granted by Lemma \ref{lAuxCompPstAlt3} %creo q esto no hace falta aqui sino solo para el paso vital de la demo
and any $\uprem \in \prem{e \cltop t}$.
\begin{itemize}
	\item $\sA{\pruD{\uprem}} \subseteq \sA{\pruD{e \cltop t}}$. % by definition
    \item If $\uprem \not\equiv e \cltop t$ then $\pruD{\uprem} \ordLex \pruD{e \cltop t}$: proper direct or indirect premises are smaller w.r.t.\ $\ordLex$.
\end{itemize}
\end{lemma}
\begin{proof}
First part holds because $\uprem \in \prem{e \cltop t}$ implies $\prem{\uprem} \subseteq \prem{e \cltop t}$, but then $\sA{\pruD{\uprem}} \subseteq \sA{\pruD{e \cltop t}}$ by definition. Concerning the second, by the first part we only have to prove that $\size{\pruD{\uprem}} < \size{\pruD{e \cltop t}}$, which is a consequence of $\uprem \in \prem{e \cltop t}$, $\uprem \not\equiv e \cltop t$. % and Lemma \ref{lAuxCompPstAlt3}. no hace falta, pq si nos referimos sin querer a una hipotesis entonces esta seguira teniendo tamaño menor
\end{proof}


From now on we will assume that every \apcrwl-proof that we consider fulfills the requirements of Lemma \ref{lAuxCompPstAlt3}. 
Now we are ready to prove Lemma \ref{lAuxCompPstAlt2}.

\begin{proof}[Proof for Lemma \ref{lAuxCompPstAlt2}]\label{PROOFlAuxCompPstAlt2}
We assume we start with a proof for $\prog \uplus \progm \pps e \cltop t$ which fulfils the conditions granted by Lemma \ref{lAuxCompPstAlt3}, and proceed by induction over $\ordLex$ applied over $\prog \uplus \progm \pps e \cltop t$. Let us do a case distinction over the rule applied at the root of the proof:
\begin{description}
 \item[B] Then $t \equiv \perp$ and $\progh \uplus \progm \vdash e \rw^0 e$ for which $\perp \ordap |e|$ holds.
 \item[RR] Then $e \equiv X \equiv t$ and $\progh \uplus \progm \vdash e \rw^0 e$ for which $X \ordap X \equiv |e|$ holds.
 \item[DC] If $e \equiv c \in \CS^0$ then $t \equiv c$ and so $\progh \uplus \progm \vdash e \rw^0 e$ for which $c \ordap c \equiv |e|$ holds. Otherwise $\prog \uplus \progm \pps e \equiv c(e_1, \ldots, e_n) \cltop c(t_1, \ldots, t_n) \equiv t$. But then by Lemma \ref{lemOrdLexExtStruct} we can apply the IH over each $\prog \uplus \progm \pps e_i \cltop t_i$ of the starting proof, thus getting $\progh \uplus \progm \vdash e_i \rw^* e'_i$ such that $t_i \ordap |e'_i|$. But then $\progh \uplus \progm \vdash e \equiv c(e_1, \ldots, e_n) \rw^* c(e'_1, \ldots, e'_n)$, for which $t \equiv c(t_1, \ldots, t_n) \ordap c(|e'_1|, \ldots, |e'_n|) \equiv |c(e'_1, \ldots, e'_n)|$.
   \item[\apor] Then we have $f(\overline{e}) \cltop t$. In case $t \equiv \perp$ lemma holds trivially for $f(\overline{e}) \rw^0 f(\overline{e})$ with $t \equiv \perp \ordap \perp \equiv |f(\overline{e})|$. Otherwise we proceed by a case distinct over $f$.\\
\underline{If $f \in \FS^\prog$} for the sake of sake of simplicity we will consider $f \in \FS^1$---the proof can be easily extended to functions with zero or more than one arguments, due to left linearity of program rules. Assume the rule used was $(f(p) \tor r) \in \prog$, so we have the following starting proof.
$$
\infer[\mbox{\apor}]{\prog \uplus \progm \vdap f(e) \clto t}
{
\begin{array}{l}
e \clto p\theta_1 \\ \ldots \\ e \clto p\theta_m
\end{array}
~~
\begin{array}{l}
~ \\ ~ \\ r?\{\theta_1, \ldots, \theta_m\} \clto t
\end{array}
}
$$
The transformed rule corresponding to $(f(p) \tor r)$ would be  $f(Y) \tor \mi{if}~\match(Y)$ $\thn~r[\overline{X_i/\prj_i(Y)}]$, where $\overline{X_i} = \mivar(p) \cap \mivar(r)$, % = var(r)$ (as $var(r) \subseteq var(p)$, because we have no extra variables in program rules),
while the rules for $\match$ and each $\prj_i$ would be $\match(p) \tor \tru$, $\prj_i(p) \tor X_i$. Then by Lemma \ref{lemOrdLexExtStruct} we can apply the IH over any $\prog \uplus \progm \vdap e \clto p\theta_j$, so we pick an arbitrary $\theta_j \in \{\theta_1, \ldots, \theta_m\}$ thus getting $\progh \uplus \progm \vdash e \rw^* e'_j$ such that $p\theta_j \ordap |e'_j|$. Then, as $p$ is linear because it is in the left-hand side of a program rule, by Lemma \ref{lAuxCompPstAlt} there must exists some $\sigma_j \in \Subst$ such that $p\sigma_j \equiv e'_j$, so we can do
$$
\begin{array}{l}
\progh \uplus \progm \vdash f(e) \rw \mi{if}~\match(e)~\thn~r[\overline{X_i/\prj_i(e)}] \\
\rw^* \mi{if}~\match(e'_j)~\thn~r[\overline{X_i/\prj_i(e)}] \\
\equiv \mi{if}~\match(p\sigma_j)~\thn~r[\overline{X_i/\prj_i(e)}] \\
\rw \mi{if}~\tru~\thn~r[\overline{X_i/\prj_i(e)}] \rw r[\overline{X_i/\prj_i(e)}] 
\end{array}
$$
Now, in order to enable the application of the induction hypothesis over $\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \clto t$ we will prove that this statement holds, and also do some calculations with $\sA{\_}$. By Lemma \ref{lAuxCompPstAlt3} we can assume a \apcrwl-proof $\pru$ for $f(e) \cltop t$ such that it is not a premise of itself, and so $\sA{\pruD{f(e) \cltop t}} = \{f(e) \cltop t\} \uplus \cjtoD$, where $\cjtoD = (\bigcup_{j \in \{1, \ldots, m\}} \sA{\pruD{e \cltop p\theta_j}}) \cup \sA{\pruD{r?\{\theta_1, \ldots, \theta_m\} \cltop t}}$. Now, if we could prove that there is a proof $\pru'$ for $\prog \uplus \progm \pps r[\overline{X_i/\prj_i(e)}] \cltop t$ such that $\sA{\pru'} \subseteq \cjtoD$, then we would have $\sA{\pru'} \subseteq \cjtoD \subset \sA{\pruD{f(e) \cltop t}}$ so we can apply the induction hypothesis to get a derivation $\progh \uplus \progm \vdash r[\overline{X_i/\prj_i(e)}] \rw^* e'$ such that $t \ordap |e'|$.

Therefore, all that is left is proving that such a proof $\pru'$ exists. To do that we proceed by induction on the structure of $r$---taking into account that $r \in \Exp$ as it is the right-hand side of a program rule---and proving that, from $\pruD{r?\{\theta_1, \ldots, \theta_m\} \cltop t}$, we can build a proof 
$\pru'$ for $\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \clto t$ under the conditions above. Regarding the base cases.
\begin{itemize}
	\item If $r \equiv Y \in \var$: in order to make the proof more solid, we will consider here the more general case where $f \in FS^n$ for any $n \geq 0$, so the starting statement is $\progh \uplus \progm \vdap f(\overline{e}) \clto t$,  the rule used is $(f(\overline{p}) \tor r) \in \prog$ and the proof $\pru'$ is being built for the statement $\progh \uplus \progm \vdap r[\overline{X_{i j}/\prj_{i j}(e_i)}] \cltop t$. Then $\{Y\} = \mivar(r) \subseteq \mivar(\overline{p})$, because of the absence of extra variables, therefore $\exists p_i \in \overline{p}. Y \in \mivar(p_i)$. But as $\overline{X_{i j}} = \mivar(p_i) \cap \mivar(r)$ we get $\exists X_{i j} \in \overline{X_{i j}}. Y \equiv X_{i j}$, as a consequence, and so $r[\overline{X_{i j}/\prj_{i j}(e_i)}] \equiv Y[\overline{X_{i j}/\prj_{i j}(e_i)}] \equiv \prj_{i j}(e_i)$. 

Going back to the case where $f \in \FS^1$, that implies that $r[\overline{X_i/\prj_i(e)}] \equiv \prj_{Y}(e)$. We will now use the hypothesis $\pruD{r?\{\theta_1, \ldots, \theta_m\} \cltop t}$ proof to find our $\pru'$. We have two possibilities.
\begin{enumerate}
	\item $\forall \theta \in \{\theta_1, \ldots, \theta_m\}. Y \in \dom(\theta)$: Then $\prog \uplus \progm \vdap r?\{\theta_1, \ldots, \theta_m\} \equiv \theta_1(Y)~?~\ldots~?~\theta_m(Y) \clto t$. But that implies that $\exists \theta_j \in \{\theta_1, \ldots, \theta_m\}. \prog \uplus \progm \vdap \theta_j(Y) \clto t$, so we can build $\pru'$ as.
$$
\infer[\mbox{\apor}]{\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \equiv \prj_{Y}(e) \clto t}
{
\infer{e \clto p\theta_j}{\hypothesis}
& \theta_j(Y) \clto t
}
$$
But $\theta_j \in \CSubst_\perp$ implies $\sA{\pruDp{\theta_j(Y) \clto t}} = \emptyset$. Besides, we have defined $\pruDp{e \clto p\theta_j}$ as $\pruD{e \clto p\theta_j}$, and $\sA{\pruD{e \clto p\theta_j}} \subseteq \cjtoD$ by definition of $\cjtoD$, therefore $\sA{\pru'} = \sA{\pruDp{r[\overline{X_i/\prj_i(e)}] \clto t}} = \sA{\pruDp{\theta_j(Y) \clto t}} ~\cup~ \sA{\pruDp{e \clto p\theta_j}} \subseteq \cjtoD$.

\item $\exists \theta_j \in \{\theta_1, \ldots, \theta_m\}. Y \not\in \dom(\theta_j)$: Then $\prog \uplus \progm \vdap r?\{\theta_1, \ldots, \theta_m\} \equiv Y~?~\rho_1(Y)~?~\ldots~?~\rho_l(Y) \clto t$, for $\{\rho_1, \ldots, \rho_l\} \subseteq \{\theta_1, \ldots, \theta_m\}$. But then, either $\exists \rho_k \in \{\rho_1, \ldots, \rho_l\}. \prog \uplus \progm \vdap \rho_k(Y) \clto t$ so we can do like in the previous case; or $\prog \uplus \progm \vdap Y \clto t$. As we discarted $t \equiv \perp$ at the beginning of the case for \apor, that implies $t \equiv Y$, so we can build $\pru'$ as.
$$
\infer[\mbox{\apor}]{\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \equiv \prj_{Y}(e) \clto Y \equiv t}
{
\infer{e \clto p\theta_j}{\hypothesis}
& \infer[\crule{RR}]{\theta_j(Y) \equiv Y \clto Y}{}
}
$$
by using that $\theta_j \in \{\theta_1, \ldots, \theta_m\}. Y \not\in \dom(\theta_j)$ above. Like in the previuos case $\sA{\pruDp{Y \clto Y}} = \emptyset$, and we can do the same computations with $\sA{\_}$ to conclude $\sA{\pru'} \subseteq \cjtoD$. 
\end{enumerate}
    \item If $r \equiv c \in \CS^0$: Then $\prog \uplus \progm \vdap r?\{\theta_1, \ldots, \theta_m\} \equiv c \clto t$ implies $t \equiv c$, because $t \not\equiv \perp$, so we can build $\pru'$ as.
$$
\infer[\crule{DC}]{\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \equiv c \clto c \equiv t}{}
$$
with $\sA{\pru'} = \sA{\pruDp{r[\overline{X_i/\prj_i(e)}] \clto t}} = \sA{\pruDp{c \clto c}} = \emptyset \subseteq \cjtoD$. 
    \item The case for $r \equiv g \in \FS^0$ is included in the general case for $g \in FS$ below. 
\end{itemize}
Concerning the inductive steps.
\begin{itemize}
	\item If $r \equiv c(a_1, \ldots, a_l)$ for $c \in \CS^l$: As $t \not\equiv \perp$ then the hypothesis must be $\prog \uplus \progm \vdap r?\{\theta_1, \ldots, \theta_m\} \equiv c(a_1?\{\theta_1, \ldots, \theta_m\}, \ldots, a_l?\{\theta_1, \ldots, \theta_m\})  \cltop c(t_1, \ldots, t_l) \equiv t$, where for each $a_k$ we have $\prog \uplus \progm \vdap a_k?\{\theta_1, \ldots, \theta_m\}$ $\clto t_k$. But then by IH over each $a_k$ we get a proof %$\pruDp{\prog \uplus \progm \vdap a_k[\overline{X_i/project_i(e)}] \clto t_k}$
$\pruDp{a_k[\overline{X_i/\prj_i(e)}] \clto t_k}$, and we can combine all these proofs together to build $\pru'$ as a proof for the statement 
$$
\begin{array}{l}
\prog \uplus \progm \vdap r[\overline{X_i/\prj_i(e)}] \\
\equiv c(a_1[\overline{X_i/\prj_i(e)}], \ldots, a_l[\overline{X_i/\prj_i(e)}]) \clto c(t_1, \ldots, t_l) \equiv t
\end{array}
$$%,
by perfoming a \crule{DC} step at the root of $\pru'$ and using each $\pruDp{a_k[\overline{X_i/\prj_i(e)}] \clto t_k}$ as hypothesis. But then $\sA{\pru'} = \bigcup_{k \in \{1, \ldots, l\}} \sA{\pruDp{a_k[\overline{X_i/\prj_i(e)}] \clto t_k}} \subseteq \cjtoD$, as for each $a_k$ we have $\sA{\pruDp{a_k[\overline{X_i/\prj_i(e)}] \clto t_k}} \subseteq \cjtoD$ by IH. 
	\item If $r \equiv g(a_1, \ldots, a_l)$ for $g \in \FS^l$: As $t \not\equiv \perp$ then the \apcrwl\ rule used at the root of $\prog \uplus \progm \vdap r?\{\theta_1, \ldots, \theta_m\} \equiv g(a_1, \ldots, a_l)?\{\theta_1, \ldots, \theta_m\} \clto t$ must be \crule{\apor}, let $r'\mu$ be the
right-hand side of the rule and the parameter passing substitution used in that step. We can proceed like in the previous case, applying the IH over each $\prog \uplus \progm \vdap a_k?\{\theta_1, \ldots, \theta_m\} \clto s_j$ getting a proof $\pruDp{a_k[\overline{X_i/\prj_i(e)}] \clto s_j}$, and then build $\pru'$ by using \crule{\apor} at the root, and $\pruD{r'\mu \clto t}$ as the last hypothesis. On one hand we have $\sA{\pruDp{a_k[\overline{X_i/\prj_i(e)}] \clto s_j}} \subseteq \cjtoD$ for each of these premises by IH. On the other hand 
$$
\begin{array}{l}
\sA{\pruDp{r'\mu \clto t}} = \sA{\pruD{r'\mu \clto t}} \\
\subseteq \sA{\pruD{g(a_1, \ldots, a_l)?\{\theta_1, \ldots, \theta_m\} \clto t}} \\
= \sA{\pruD{r?\{\theta_1, \ldots, \theta_m\} \clto t}} \subseteq \cjtoD
\end{array}
$$
therefore $\sA{\pru'} \subseteq \cjtoD$.
\end{itemize}

\underline{If $e \equiv \match(e_1, \ldots, e_n)$ } for some of these auxiliary $\match$ functions in ${\cal M}$, with rule $\match(p_1, \ldots, p_n) \tor \tru$, then as $t \not\equiv \perp$ we have $t \equiv \tru$ with:
$$
\infer[\crule{POR}]{\prog \uplus \progm \pps e \equiv \match(e_1, \ldots, e_n) \cltop \tru}
          {
           e_1 \cltop p_1\theta_1
        & \ldots
        & e_n \cltop p_n\theta_n
        & \tru \cltop \tru
            }
$$
There could be more evaluations for each $e_i$ but those are useless because $\tru$ is ground. Then by Lemma \ref{lemOrdLexExtStruct} we can apply the IH over each $\prog \uplus \progm \pps e_i \cltop p_i\theta$ so we get 
%Then we have $\pruD{e_i \cltop p_i\theta_i} \ordLex \pruD{e \cltop \tru}$ as we saw before, hence by IH 
$\progh \uplus \progm \vdash e_i \rw^* e'_i$ such that $p_i\theta_i \ordap |e'_i|$. But then by Lemma \ref{lAuxCompPstAlt} there must exist some $\sigma_i \in Subst$ such that $p_i\sigma_i \equiv e'_i$, and we can do $\progh \uplus \progm \vdash match(e_1, \ldots, e_n) \rw^* match(e'_1, \ldots, e'_n) \equiv match(p_1\sigma_1, \ldots, p_n\sigma_n) \rw \tru$, and $\tru \ordap \tru \equiv |\tru|$.\\


\underline{If $e \equiv \prj(e_1)$} for some of these auxiliary functions, with rule $\prj(p) \tor X$, then as $t \not\equiv \perp$ we have:
$$
\infer[\crule{POR}]{\prog \uplus \progm \pps e \equiv \prj(e_1) \cltop t}
           {
            \begin{array}{l} e_1 \cltop p\theta_1 \\ \ldots \\ e_1 \cltop p\theta_m \end{array}~
           \ \begin{array}{l} ~ \\ ~ \\ X(?\{\theta_1, \ldots, \theta_m\}) \cltop t \end{array}~
          }
$$
Then there must exist some $\theta_j \in \{\theta_1, \ldots, \theta_m\}$ such that $X\theta_j \cltop t$, hence $t \ordap \theta_j(X)$ by Lemma \ref{lSimplePropPCRWL}. %Besides we have $\pruD{e_1 \cltop p\theta_j} \ordLex \pruD{e \cltop t}$ as we saw before, hence by IH 
But then by Lemma \ref{lemOrdLexExtStruct} we can apply the IH over $\prog \uplus \progm \pps e_1 \cltop p\theta_j$ so we get 
$\progh \uplus \progm \vdash e_1 \rw^* e'_j$ such that $p\theta_j \ordap |e'_j|$, to which we can apply Lemma \ref{lAuxCompPstAlt} to get some $\sigma_j \in \Subst$ such that $p\sigma_j \equiv e'_j$ and $\theta_j \ordap \sigma_j$. Therefore $t \ordap \theta_j(X) \ordap \sigma_j(X)$, so it is trivial to check that then $t \ordap |\sigma_j(X)|$ (by induction on the structure of $t$), and we can do $\progh \uplus \progm \vdash \match(e_1) \rw^* \match(e'_j) \equiv \match(p\sigma_j) \rw \sigma_j(X)$.\\

\underline{If $e \equiv if~e_1~then~e_2$} then as $t \not\equiv \perp$ we have:
$$
\infer[\crule{POR}]{\prog \uplus \progm \pps e \equiv \mi{if}~e_1~\thn~e_2 \cltop t}
           {
           \begin{array}{l} ~ \\ ~ \\e_1 \cltop \tru\end{array}~
          \   \begin{array}{l} e_2 \cltop t_1 \\ \ldots \\ e_2 \cltop t_m\end{array}~
          \ \begin{array}{l} ~ \\ ~ \\t_1? \ldots? t_m \cltop t\end{array}~
           }
$$
There could be more evaluations for $e_1$ but those are useless because $\tru$ is ground. 
But then by Lemma \ref{lemOrdLexExtStruct} we can apply the IH over $\prog \uplus \progm \pps e_1 \cltop \tru$ so we get 
%We have $\pruD{e_1 \cltop \tru} \ordLex \pruD{e \cltop t}$ as we saw before, hence by IH 
$\progh \uplus \progm \vdash e_1 \rw^* e'_1$ such that $\tru \ordap |e'_1|$. Then we can apply Lemma \ref{lAuxCompPstAlt} to get some $\sigma_1 \in Subst$ such that $\tru \equiv \tru\sigma_1 \equiv e'_1$, so we can do $\progh \uplus \progm \vdash \mi{if}~e_1~\thn~e_2 \rw^* \mi{if}~e'_1~\thn~e_2 \equiv \mi{if}~\tru~\thn~e_2 \rw e_2$. Besides $t_1? \ldots? t_m \cltop t$ implies $t_j \cltop t$ for some $t_j \in \{t_1, \ldots, t_m\}$ such that $t \ordap t_j$, by Lemma \ref{lSimplePropPCRWL}. % and $\pruD{e_2 \cltop t_j} \ordLex \pruD{e \cltop t}$ as we saw before. We can apply the IH to get 
But then by Lemma \ref{lemOrdLexExtStruct} we can apply the IH over $\prog \uplus \progm \pps e_2 \cltop t_j$ so we get 
$\progh \uplus \progm \vdash e_2 \rw^* e'$ such that $t \ordap t_j \ordap |e'|$.\\

\underline{If $e \equiv e_1~?~e_2$ }then as $t \not\equiv \perp$ we have $e_i \cltop t$ for some $i \in \{1, 2\}$ with a proof to which we can apply the IH by Lemma \ref{lemOrdLexExtStruct} to get $\progh \uplus \progm \vdash e_1~?~e_2 \rw e_i \rw^* e'$  such that $t \ordap |e'|$.
 \end{description} 
\end{proof}

\subsection{For Section \ref{subsec:logics}}
\begin{theorem}[Compositionality of \sapcrwl\ and \sbpcrwl]\label{lCompPSMix} 
For any program, $\con \in \Cntxt$ and $e, e' \in \Exp_\perp$:%, 
$$
\begin{array}{c}
\densap{\con[e]} = \bigcup_{\{t_1, \ldots, t_n\} \subseteq \densap{e}} \densap{\con[t_1~?~\ldots~?~t_n]} \\
\densbp{\con[e]} = \bigcup_{\{t_1, \ldots, t_n\} \subseteq \densbp{e}} \densbp{\con[t_1~?~\ldots~?~t_n]}
\end{array}
$$
%, 
for any arrangement of the elements of $\{t_1, \ldots,$ $t_n\}$ in $t_1~?~\ldots~?~t_n$. As a consequence:
$$
\begin{array}{c}
\densap{e} = \densap{e'} \mbox{ iff  } \forall \con \in \Cntxt. \densap{\con[e]} = \densap{\con[e']} \\
\densbp{e} = \densbp{e'} \mbox{ iff  } \forall \con \in \Cntxt. \densbp{\con[e]} = \densbp{\con[e']} 
\end{array}
$$
\end{theorem}
\begin{proof}
A straightforward modification of the proof for Theorem \ref{lCompPS}.
\end{proof}

\begin{proposition}[Compositionality of \sapcrwl\ and \sbpcrwl\ for singular contexts]\label{lemCompSPlsSingCon}
For any program, singular context $\scon$ and $e \in \Exp_\perp$:
$$
\begin{array}{c}
\densap{\scon[e]} = \bigcup\limits_{t \in \densap{e}} \densap{\scon[t]} \\
\densbp{\scon[e]} = \bigcup\limits_{t \in \densbp{e}} \densbp{\scon[t]} \\
\end{array}
$$
\end{proposition}
\begin{proof}
Again, a straightforward modification of the proof for Theorem \ref{lCompPS}.
\end{proof}

\begin{proposition}[Bubbling for singular contexts in \sapcrwl\ and \sbpcrwl]\label{bubSPlurals}
For any program, singular context $\scon$ and $e_1, e_2 \in \Exp_\perp$:
$$
\begin{array}{c}
\densap{\scon[e1~?~e_2]} = \densap{\scon[e_1]~?~\scon[e_2]} \\
\densbp{\scon[e1~?~e_2]} = \densbp{\scon[e_1]~?~\scon[e_2]}
\end{array}
$$
\end{proposition}
\begin{proof}
A straightforward adaptation of the proof for Proposition \ref{bubAPlural}.
\end{proof}
